Towards Self-Tuning Parameter Servers

Recent years, many applications have been driven advances by the use of Machine Learning (ML). Nowadays, it is common to see industrial-strength machine learning jobs that involve millions of model parameters, terabytes of training data, and weeks of training. Good efficiency, i.e., fast completion time of running a specific ML job, therefore, is a key feature of a successful ML system. While the completion time of a long-running ML job is determined by the time required to reach model convergence, practically that is also largely influenced by the values of various system settings. In this paper, we contribute techniques towards building self-tuning parameter servers. Parameter Server (PS) is a popular system architecture for large-scale machine learning systems; and by self-tuning we mean while a long-running ML job is iteratively training the expert-suggested model, the system is also iteratively learning which system setting is more efficient for that job and applies it online. While our techniques are general enough to various PS-style ML systems, we have prototyped our techniques on top of TensorFlow. Experiments show that our techniques can reduce the completion times of a variety of long-running TensorFlow jobs from 1.4x to 18x.

==> 0-Online.tex <==
%!TEX root = 0-paper.tex

%
\section{Online Job Optimization Framework}
\label{tuning}
%Let's begin with an overview of PSTuner.
Figure \ref{fig:system} shows our proposed framework to carry out online ML job optimization.
In this paper, we endeavor to devise off-the-shelf techniques that could be integrated with as many existing ML systems as possible.
Therefore, the framework aims to reuse the ML system front-end
so that ML users do not need to learn a new API
but can enjoy the completion time speedup brought by auto-tuning.

\begin{figure}
\centering
\includegraphics[width=8cm]{images/system}
\caption{Online job optimization framework}
\label{fig:system}
\end{figure}

%On receiving a
%
%
%Installing PSTuner would not change the front-end of the target ML system, which parses the input ML program $P$ and creates a process for that job. %\footnote{In TensorFlow, the front-end also extracts the configuration $c$ from the program $P$.}
On receiving an ML job $J$ from the front-end,
the job will be \emph{instrumented} as $J'$ before sending to the ML system back-end
so that it would emit various  \emph{per-iteration} metrics (e.g., execution time, loss) to a repository during its execution.
%
%
%
%PSTuner will insert certain \emph{instrumentation} code to the job and then pass the instrumented job $J'$ to the target ML system back-end for execution.
%On finishing an iteration, the instrumentation code will write the execution metrics (e.g., the execution time and the loss) of that iteration into PSTuner's repository.
Before starting an iteration, the \emph{Tuning Manager} will (1) update a statistical model based on the newly collected metrics,
(2) recommend a new configuration of system setting $X'$, and (3) reconfigure the system to setting $X'$.
%As we illustrate momentarily,
%we will develop \emph{non-quiescent} techniques to %carry out \emph{live reconfiguration}
%%in order to reduce the blocking time between reconfiguration overhead.
%%One of them is the \emph{lazy strategy}
%%that pushes/pulls the parameters to/from the new destinations/sources
%hide the system reconfiguration delay in an iteration.   % inside an iteration.
%As a result,
%on receiving a new configuration $X'$,
%the \emph{Reconfiguration Manager} of PSTuner will insert certain \emph{reconfiguration} code to the job and
%start the next iteration.
%Despite the reduced reconfiguration cost,
Practically,  the Tuning Manager might not return a new recommendation after every iteration
but execute a certain number of iterations for each setting in order to understand its statistics efficiency (e.g., the live convergence rate).
%On the other hand, that further avoids the reconfiguration overhead.
%In the following, we briefly discuss the Tuning Manager
%and the Reconfiguration Manager.  We end this section with our Research Agenda.


%
%
%As mentioned, we deliberately aim to integrate PSTuner with open-source ML software libraries
%so that our potential users do not need to learn a new API or modify their existing ML programs but can enjoy the self-driving feature.
%Although the techniques that we will develop are general,
%we use TensorFlow, an open-source ML framework developed by Google, as an example to demonstrate how PSTuner integrates with it.
%For TensorFlow, the system configuration is embedded inside the ML program.
%PSTuner will start with using TensorFlow's front-end to extract the system configuration $c$ from the program.
%Then, PSTuner's {\bf scheduler} will execute the first iteration based on the given system configuration $c$.
%The scheduler will collect the execution metrics after each iteration (e.g., the execution time and the loss/error) and insert them into a repository.
%Next, PSTuner's {\bf online tuner} will (1) update its ML model based on the newly collected metrics,
%and when appropriate  (2) recommend a new configuration $c'$ and (3) apply the new reconfiguration.
%Finally, the scheduler will start a new iteration.
%

\subsection{Problem Formulation}\label{problem}
Given an ML job $J$, one key goal of the tuning manager is to find the optimal or near-optimal system setting $X^*$ that minimizes the {remaining} completion time.
Let $ X  = \langle c_1 = v_1, \dots, c_d = v_d\rangle$ be a system setting,
where each $c_i$ is a configurable system parameter with value $v_i$.
%We use $X_i$ to denote the setting being used at a particular moment $\loss$
We use $\T(\langle X, \loss_j \rangle)$ to denote the remaining completion time of the job
if we switch to setting $X$
%after the $j$-th iteration,
where the model has reached a loss down to $\loss_j$.
$\langle X, \loss_j \rangle$ is simply a $(d+1)$-dimensional vector that includes both the system setting values and the loss of the model.
%after the model parameter has been updated to $\w_j$.

%at moment $\loss$.
%Along the iterations of the job,
%we can collect data like:
%
%$$\langle \loss_0, X_0, T(X_0, \loss_0) \rangle, \dots, \langle \loss_m, X_m, T(X_m, \loss_m) \rangle$$

Then, %formally, %at another particular moment $\loss'$,
the problem is, given a model whose loss is $\loss_j$,
find the $X$ that minimizes $\T(\langle X, \loss_j \rangle)$.
Knowing $\T(\langle X, \loss_j \rangle)$ ahead would be infeasible.
% but it requires all candidate settings to be tried.\footnote{One may wonder
%whether we can \emph{simulate}  instead of actual \emph{execute} in order to approximate $T_\loss(X)$ at (almost) no cost,
%as in \cite{BabuSOCC10}.
%Unfortunately that idea can't transfer to here ---
%while a simulation may give good estimates on the hardware efficiency,
%it cannot tell anything about the statistical efficiency (e.g., the loss) of an iteration unless it carries out the computation using the real data.}
Therefore, we employ Bayesian Optimization (BO) \cite{BOTutorial, BONIPS2012,BAGO}  to search for an approximation solution with significantly smaller cost.
In what follows, we drop $X$ and $\loss_j$ if the context is clear and represent $\T(\langle X, \loss_j \rangle)$ as $T$.


\subsection{Bayesian Optimization}
Bayesian Optimization (BO) is a strategy for optimizing a  black-box objective function  that is unknown beforehand but  observable through conducting experiments,
like our $\T$.
By modeling $\T$ as a Gaussian Process \cite{gp},
BO can return an estimate of $\T$ given any $X$ and $\loss$.
%based on collecting experimental observations: $\langle \loss_0, X_0, T_0 \rangle$, $\dots$, $\langle \loss_m, X_m, T_m \rangle$.
The estimate and its confidence interval
would progressively improve with the number of observations.


BO has the ability to suggest the next setting
using a pre-defined \emph{acquisition function} that also gets updated with more observations.
There are many choices of {acquisition function}
such as (i)  Probability of Improvement (PI) \cite{BONIPS2012}, which picks the next setting that can maximize the probability of improving the current best;
(ii) Expected Improvement (EI) \cite{gp}, which picks the next setting that can maximize the expected improvement over the current best;
(iii) Upper Confidence Bound (UCB) \cite{GPUCB}, which picks the one that has the smallest lower bound in its certainty region.
Different acquisition functions
have different strategies to balance between \emph{exploring} $\T$ (so that it tends to suggest a setting in an unknown region of the response surface)
and \emph{exploiting} the  knowledge so far (so that it tends to suggest a setting that lies in a known high performance region).
In this paper, we choose EI because it has shown to be more robust than PI, and unlike UCB, it is parameter-free.
Using BO with EI has the ability to learn the objective function quickly and always return the expected optimal setting.

BO itself is noise resilient.  Specifically,
what we can collect from experiments is actually $\T'$:



\begin{equation}
\T' = \T  + e
\end{equation}

\noindent
where $e$ is a Gaussian noise with zero mean, i.e., $e \sim \mathbb{N}(0, \sigma^2)$.
Since $\T'$, $\T$, and  $e$ are Gaussian,
we can infer $\T$ and its confidence interval~\cite{cherrypick}.
As we will discuss in Section \ref{progress},
the observation noise comes from the fact $\T'$ is not a direct measurement
but a product between (i) \emph{per-iteration execution time} (hardware efficiency)
and (ii) \emph{estimated number of iterations left} (statistical progress).
Although (i) could be directly observed,
(ii) has to be based on turning a theoretical bound into an estimate based on the current progress (Section \ref{progress}).

There are also some other reasons that we choose BO.
First, BO has an advantage of being {non-parametric},
meaning it does not impose any limit on $\T$, making
our techniques useful for a variety of ML systems and platforms (system agnostic).
Furthermore, it
can deal with non-linear response surface but require far fewer samples  (quick learner with confidence) than others with similar power like deep network.
Lastly, BO has a good track record on tuning database systems \cite{ituned,andyMLtune}.

In the following, we briefly describe how to model $\T$ as a Gaussian Process (GP).
For details about GP, we refer readers to \cite{gp}.
In a nutshell, GP models $\T(\langle X, \loss_j \rangle)$ by a mean function $m(\cdot)$ and a covariance kernel function $k(\cdot,\cdot)$:

\begin{eqnarray*}
m(\langle X_i, \loss_i \rangle)& =  & \mathbb{E}[\T(\langle X_i, \loss_i \rangle)]   \\
m(\langle X_j, \loss_j \rangle)& =  &\mathbb{E}[\T(\langle X_j, \loss_j \rangle)]   \\
k(\langle X_i, \loss_i\rangle , \langle X_j, \loss_j\rangle)& = & \mathbb{E}[(\T(\langle X_i, \loss_i \rangle) - m(\langle X_i, \loss_i \rangle)) \\
         &      &(\T(\langle X_j, \loss_j \rangle) - m(\langle X_j, \loss_j \rangle))]
\end{eqnarray*}

\noindent
where the kernel function makes sure $\T(\langle X_i, \loss_i \rangle)$ and  $\T(\langle X_j, \loss_j \rangle)$ have large covariance if $\langle X_i, \loss_i \rangle$ and $\langle X_j, \loss_j \rangle$ are similar
and have small covariance otherwise.
In this work,
we adopt Mat\'{e}rn covariance \cite{MCFunction} as the kernel function because it does not require strong smoothness.

There is a closed-form for the EI acquisition function from \cite{jones}.
Let $t$ be the minimum value of $T$ observed
from the current best setting so far.
For each candidate setting $X$ and a model with loss $\loss$, we can compute its \emph{expected improvement} of using $X$ (over the current best known setting) as:

\[ EI(\langle X, \loss\rangle)  =  \left \{ \begin{array}{rl} (t - m(\langle X, \loss\rangle))\Phi(Z) + \sigma(\langle X, \loss \rangle)\phi(Z)  & \text {if~}  \sigma(X_i) > 0 \\ 0 & \text {if~}  \sigma(X_i) = 0   \end{array} \right.
\]

\noindent
$\sigma(\langle X, \loss \rangle) = \sqrt{k(\langle X, \loss\rangle , \langle X, \loss\rangle)}$,
$Z = \frac{t - m(\langle X, \loss\rangle)}{\sigma(\langle X, \loss \rangle)}$, and $\Phi$ and $\phi$ are the CDF and PDF of standard normal, respectively.




%%
%%Now, before we move on, let's first explain our rational of using Machine Learning, specifically, using GPR:
%%
%%\begin{itemize}
%%\item The use of machine learning makes PSTuner \emph{system agnostics}.
%%Specifically, we don't need to understand the meaning of each individual system knob,
%%enabling PSTuner's key techniques easily adopt to different PS-style ML systems.
%%%Also, the use of ML makes PSTuner \emph{resource agnostics},
%%%letting PSTuner can easily adopt to cluster with heterogenous machines or with other co-running systems (e.g., Spark).
%%
%%\item GPR is a state-of-the-art technique with power approximately equal to that of deep networks
%%but it is far less  computationally expensive and requires far less training data while offering confidence intervals.
%%Furthermore, since it is non-parametric, it does not need any pre-defined format for the performance model.
%%%Lastly, as a probabilistic model it estimates a confidence interval, which is extremely helpful with few training examples.
%%%\item GPR is a probabilistic model with a known distribution (Guassian), enabling us to derive a closed-form for $\EIP(X)$.
%%\item %When working with our candidate setting selection strategy that picks a candidate setting with the maximum $\EIP$,
%%%GPR  offers confidence interval
%%%to quantify the uncertainty region of the performance model.
%%%It thereby can guide the search even in face of model inaccuracy.
%%GPR is easily updatable with new data.
%%Also, when working with $\EIP$,
%%it has the ability to learn the response surface quickly and only explore the areas that most likely contain the minimal \cite{cherrypick}.
%%%naturally balances between exploring an unknown region to find the global optimal and exploiting a known high performance region to find a  better local optimal.
%%%
%%%naturally balances the tasks of exploration (understanding the response surface)
%%%and exploitation (going after known low-completion-time regions).
%%%When learning, GPR ``trusts'' the result from similar configurations more (through the covariance function), and the variance for those data points decreases.
%%%The expected improvement is near-zero at sampled points and increases marginally in between them.  Thus, it always returns a setting that it believes is optimal or one that it knows little about.
%%Over time, the quality of the recommendation increases
%%%along the iterations.
%%%expected improvement in the model drops
%%as the number of unknown regions decreases.
%%
%%%BO estimates a confidence interval (the range that the actual value should fall in with high probability) of the cost and running time under each candidate cloud configuration. The confidence interval is improved (nar- rowed) as more samples become available.
%%
%%\end{itemize}
%%
%%
%%%In this project, we attempt to use Gaussian Process Regression (GPR) \cite{gp} to recommend the next configuration. % as our first attempt.  %s that it believes will shorten the remaining completion time.
%%%%Suppose $n$ iterations have been run at settings $X^i$ so far,  where $1 \le i \le n$.
%%%Figure \ref{fig:d}a shows some example raw training data we will have right after $m$ configurations have been tried through $n$ iterations.
%%%Figure \ref{fig:d}b shows the training data after \emph{normalized} by the Tuning Manager.
%%%Specifically, the Tuning Manager tries to infer the \emph{remaining completion time} $y_i$ the job will need if it
%%%switches to using $X_i$ starting from the next iteration.
%%%These normalized data $\langle X_i, y_i \rangle$ would be the training data of  the GPR.
%%%
%%%
%%%%
%%%%normalization process aims to quantity the goodness of a setting $X^i$
%%%%by estimating the remaining completion time $y_i$ it needs, if we
%%%%%assuming $X^i$ is used from the first iteration till the model converges.
%%%%At this moment, we first defer the discussion of how to get $y_i$.
%%%
%%%
%%%
%%%
%%%
%%%
%%%
%%%%Let $y_i$ be the \emph{remaining completion time} of the job under setting $X_i$. (We defer the discussion of how to find $y_i$ at this moment.)
%%%%
%%%%$\ya$ be the execution time (\underline{h}ardware efficiency)   and $\yb$ be the loss\footnote{It is also known as the \emph{error} or the \emph{cost} in some literature.  In this proposal, we regard the loss as a function like negative log-likelihood or residual sum of squares.} (\underline{s}tatisical efficiency) of the $k$-th iteration under setting $X^i$.
%%%%After the $k$-th iteration, %the data collected so far are $\langle X^i, y^i_h, y^i_s \rangle$,
%%%%the remaining completion time $y^k$ is a function  of the hardware efficiency, statistical efficiency, and the number of iterations $k$ that have already been executed
%%%%under setting $X^i$:
%%%%
%%%%$$y^i = y(\ya, \yb, n)$$
%%%The GPR can guide PSTuner what setting it shall use next.
%%%Specifically, PSTuner can choose to stick with the current setting $X^m$,
%%%switch to the best setting seen so far $X^*$, or try a new setting.
%%%Ideally, the next setting $X'$ shall result in a $y$ that yields the maximum \emph{improvements} $\IP$ over the currently best setting $X^*$ whose $y^*$ is currently minimal:
%%%
%%%\[ \IP(X)  =  \left \{ \begin{array}{rl} y^* - y  & \text {if~}  y < y^* \\ 0 & \text{otherwise}  \end{array} \right.
%%%\]
%%%
%%%
%%%$$X' = \argmax \IP(X) $$
%%%
%%%%$$X^{next} = \argmax IP(X) = \argmax (y^* - y) $$
%%%Unfortunately, %unless we have the full response surface and directly search for the optimum,
%%%$y$ is an unknown until an iteration based on $X$ is really executed.
%%%Therefore, we aim for the \emph{expected improvement} $\EIP(X)$ instead.
%%%That is, the setting $X$ that gives the \emph{maximum expected improvement} is chosen as the recommended configuration for the next iteration.
%%%%
%%%%The execution metrics collected in the previous $n$ iterations can help us to compute $\EIP(X)$ in GPR.
%%%Specifically, let $Y_X$ be a random variable representing our estimate of $y$ under setting $X$.  % based on a collected samples of $\langle X^i, y^i \rangle$.
%%%The distribution of $Y_X$ captures the uncertainty in the actual value of the remaining completion time if switching to setting $X$ in the next iteration.
%%%Let $f(p)$ be the probability density function (PDF) of $Y_X$, then:
%%%
%%%$$\EIP(X) = \int^{p=\infty}_{p=-\infty} \IP(X) f(Y_X=p) dp$$ %=  \int^{p=y(X^*)}_{p=-\infty} (Y^* - p) f(p) dp $$
%%%
%%%$$X' = \argmax \EIP(X) $$
%%%
%%%
%%%
%%%Now, the challenge boils down to estimating $y$ based on the normalized training data
%%%$\langle X^i, y^i \rangle$ available so far.
%%%Here we follow the model-driven approach in \cite{sensor} and model $y$ using GPR.
%%%Specifically, a GPR addresses the question of predicting the value of a response variable $y$,
%%%given a new input vector $X$,  and the training data.
%%%Recall that one kind of linear regression model is of the form
%%%$y = X^T\beta + \varepsilon$, where $\varepsilon \sim N(0, \sigma^2)$.
%%%The error variance $\sigma^2$ and the coefficient $\beta$ are estimated from the data.
%%%A GPR model explains the response by introducing Guassian Process (GP) latent variables
%%%$f(X_1), f(X_2), \dots, f(X_m)$, for each observation $X_i$,
%%%and explicit basis functions, $h$.
%%%A GP itself is a set of random variables, such that any finite number of them have a joint Guassian distribution.
%%%If $\{f(X), X\in \mathbb{R}^d\}$ is a GP,
%%%then given $m$ observations $X_1, X_2, \dots, X_m$, the joint distribution of the random variables
%%%$f(X_1), f(X_2), \dots, f(X_m)$ is Gaussian.
%%%A GP is defined by its mean function $M(x)$ and covariance kernel function $C(x,x')$.
%%%That is, if $\{f(X), X\in \mathbb{R}^d\}$ is a GP, then $E(f(X)) = M(X)$ and $Cov[f(X), f(X')] = E[\{f(X) - M(X)\}\{f(X') - M(X') \}] = C(X, X')$.
%%%Now consider the model:
%%%
%%%$$h(X)^T\beta + f(X)$$
%%%
%%%\noindent
%%%where, $f(X) \sim GP(0, C(X,X'))$, i.e., $f(X)$ are from a zero-mean GP with covariance function $C(X,X')$;
%%%and $h(X)$ are a set of explicit basis functions that transform the original feature vector $X$ in
%%%$\mathbb{R}^d$
%%%into a new feature vector $h(X)$ in $\mathbb{R}^k$.
%%%$\beta$ is a $k$-by-1 vector of basis function coefficients.
%%%When training the GPR model, the basis function coefficients $\beta$, the noise variance  $\sigma^2$, and the parameters of the kernel function are learned from the training data.
%%%After that, we can predict $y_i$ of any valid system configuration $X_i$ by:
%%%
%%%$$P(y_i | f(X_i), X_i) \sim N( h(X_i)^T\beta + f(X_i), \sigma^2)$$
%%%
%%%\noindent
%%%hence, the random variable $Y_{X_i}$  is a Guassian with mean equals to $h(X_i)^T\beta + f(X_i)$ and variance $\sigma^2$,
%%%meaning that we can follow \cite{jones} to derive a closed form for $\EIP$.
%%%%the probability density function $f(p)$  of $Y_X$ is the pdf of Guassian
%%%%Since $Y_{X_i}$ has a beautiful known distribution, we can derive the closed-form for $\EIP$.

%\noindent\underline{\emph{How do we generate the set of candidate settings?}}
%The GPR can give us a reliable estimate of the remaining completion time of a candidate system setting $X^{cand}$.
%However, it is also an important to discuss how do we generate the candidates.


\begin{figure}\centering
\scalebox{1.0}{
 \begin{tabular}{ccc}
   \begin{tabular}{c}
$\langle j , X_i, \ya, \yb\rangle$ \\\hline\hline
$\langle 0, X_0, t^0_0, l^0_0 \rangle$ \\
\dots  \\
$\langle 4, X_0, t^4_0, l^4_0 \rangle$ \\
$\langle 5, X_1, t^{5}_1, l^{5}_1 \rangle$ \\
\dots  \\
$\langle 9, X_1, t^{9}_1, l^{9}_1 \rangle$ \\
\dots  \\
$\langle n, X_{m}, t^{n}_m, l^{n}_m \rangle$ \\
   \end{tabular}
         &&
%   \begin{minipage}{5cm}
   \begin{tabular}{c}
$\langle X_i, \loss_i, Y_i\rangle$ \\\hline\hline
$\langle X_0, \loss_0, Y_0 \rangle$ \\
$\langle X_1, \loss_1, Y_1 \rangle$ \\
$\langle X_2, \loss_2, Y_2 \rangle$ \\
\dots  \\
$\langle X_{m}, \loss_m, Y_m \rangle$ \\
 \\
 \\
 \\
   \end{tabular}
%   \end{minipage}

    \\
   (a) collected execution metrics & & (b) training data
  \end{tabular}
  }
\caption{Execution metrics and training data}
\label{fig:d}
\end{figure}


\subsection{Using BO in Online Tuning}\label{bo}
We propose to divide the execution of an ML job into two phases: \emph{initialization} and \emph{online tuning}.

\stitle{Initialization Phase}
The \emph{initialization} phase refers to the early iterations of the job.
Its goal is to quickly bring in a small set of representative settings and their execution metrics to set up the BO.
Initially,
the job starts the first $a$ iterations using the setting $X_0$, which is the default or the one given by the user.
Iterations after that will select the one with the highest expected improvement $EI$,
from an initial \emph{orthogonal sample} $\mathcal{S}$ \cite{os} of candidate settings from the setting space.
Orthogonal sampling is chosen over
random sampling because the latter is often ineffective when only a few samples are collected from a fairly high dimensional space.
%In contrast, orthogonal sampling is an efficient method that guarantees that each subspace is evenly sampled
So, assume the initial sample size is $m$
and each setting runs $a$ iterations, the first $a + m \cdot a$ iterations belong to the initialization phase.
Figure \ref{fig:d}a illustrates the execution metrics that would be inserted into the repository after trying $m$ different settings,
with $a=5$ iterations.
Each record in the collected execution metrics is a quadruple
$\langle j , X_i, \ya, \yb\rangle$,
with
$X_i$ indicates that iteration $j$ was executed using setting $X_i$,
\ya indicates the  execution time of that iteration,
and \yb indicates the loss of the model after that iteration.
Hereafter, we also refer $\yb$ as ``the loss of iteration $j$'', which is:

\begin{equation}\label{loss}
 \yb = f(\w{}^j)-f(\w{}^*)
\end{equation}

\noindent
where $f$ is the learning function specified in the expert-suggested model (e.g., the labeling function, in classification),
 $\w{}^*$ is the optimal model parameter (while $\w{}^*$ is unknown, $f(\w{}^*)$ is known from the ground truth, e.g., the labels of the training data),
and $\w^j$  is the updated model parameter after this iteration $j$.

%$f(\w{}^*)$ is the minimum of $f(\w{}), \forall \w{} \in \mathbb{R}^n$

The loss of \emph{one} iteration alone is insufficient to judge whether a setting has good statistical efficiency.  Furthermore,
even a lousy setting could improve the loss a lot in early iterations whereas an optimal setting could hardly improve the loss if it is applied in late iterations.
Consequently, the execution metrics would be preprocessed into triples
$\langle X_i, \loss_i, Y_i\rangle$,
where $\loss_i$ is the loss of the \emph{first} iteration of using setting $X_i$, i.e., $\loss_i = l_i^{ia}$ (e.g.,  $l^0_0$, $l^{5}_1$ in Figure \ref{fig:d}a),
 and $Y_i$ is the estimated remaining completion time
assuming that the remaining iterations will use $X_i$ and \underline{resume} from where the model has reached a loss down to $\loss_i$.
We set $l_i^{ia}$ as $\loss_i$, but not or any other values like
$l_i^{(i+1)a-1}$ (i.e., the loss of the last iteration of using setting $X_i$; e.g., $l^4_0$, $l^{9}_1$ in Figure \ref{fig:d}a),
because BO is going to predict
what setting it shall use if it \underline{picks up} the job from a model whose loss is $l_i^{ia}$.
Figure \ref{fig:d}b shows the training data after preprocessing.

%
%It is also the case when BO recommend the next best setting $X_next$, more specifically, in recommendation phase, BO will estimate the remaining time to converge of each setting $X$ with moment $\loss_j$, then return the best as the recommended setting.
%Looking back, when we define $T_\loss(X)$
%as ``the remaining completion time of the job if we switch to setting $X$ at moment $\loss$'' in Section \ref{problem},
%$\loss$  essentially refers to loss  $\loss_i$ here.
%Looking back, when we define
% $\T(\langle X, \loss_j \rangle)$ as ``the remaining completion time of the job
%if we switch to setting $X$
%after the $j$-th iteration'' in Section \ref{problem},
%
%where the model has an updated loss being $\loss_j$.


The initialization phase takes a total of $n = a + m\cdot a$ iterations
and it ends with feeding all training data to the BO (i.e., to learn $\sigma$, parameter values of the kernel function, etc.).
After that is the \emph{online tuning} phase.

\stitle{Online Tuning Phase}
In this phase, a new set of orthogonal sample $S$ will be generated at the beginning of every $a$ iterations.
The set of candidate settings at the beginning of those iterations
would then be  $S \cup \mathbb{X}$,
where $\mathbb{X}$ is the set of settings that has been selected by BO and \emph{executed} so far.
Then, the next recommended setting $X'$  is the one with the highest $\EIP$:

$$X' = \argmax_{X \in S \cup \mathbb{X}} \EIP(\langle X, \loss_j\rangle)$$

Note that the sample size $S$ in the online tuning phase can be way larger than the size of the initial sample $\mathcal{S}$ %in the initialization phase
because the EIs in this phase
are obtained through calculation but not actual execution.
Furthermore, depending on the reconfiguration cost $R_{cost}$ (Section \ref{reconfig}),
a reconfiguration only happens when $\EIP(\langle X', \loss_j\rangle) - R_{cost} > 0$.
In other words, if a reconfiguration costs more than it will potentially save, that reconfiguration would not take place.
Overall, the online tuning phase goes on until the job finishes.

%One straightforward approach is to random sample a set of candidate settings from the space of valid parameter values.
%However, random sampling is often ineffective to cover the whole space when we demand fewer samples from a fairly high dimensional space.
%Therefore, in this project, we will investigate the use of \emph{Orthogonal Sampling} \cite{os} in initialization.
%Orthogonal sampling is a lightweight method that guarantees that each subspace is evenly sampled.


\stitle{Values of $a$ and $m$}
We end this section by discussing  how to set the values of $a$ and $m$.
Our major purpose is to avoid our techniques being parametric if possible.
The main usage of $a$ is to deduce the statistical progress (convergence rate). % under a setting with possibly asynchronous updates from workers.
So, we set $a$, the number of iterations executed for each setting, be the number of workers so as to assume that each worker has already pushed  the update to the server at least once, by default.
We discuss how that default value can be overridden based on the application's semantic in Section \ref{reconfig}.
Nonetheless, we remark that no systems can reach 100\% parameter-free.
For example, OtterTune, iTuned, and this paper also at least need to specify $m$, the initial sample size.
While the initial sample size used in Ottertune is unclear, iTuned evidences that a very small sample size is enough.
In this paper, we adopt $m=20$.
In Section \ref{conclusion}, we put down interesting directions about how to possibly eliminate this very last knob by \emph{transfer learning} \cite{PanY10}.




==> 0-Progress-Bo.tex <==
%!TEX root = 0-paper.tex

\begin{figure*}[ht]
	\begin{center}
    \begin{tabular}{ccc}
    \includegraphics[width=0.65\columnwidth]{images/online_1} & \includegraphics[width=0.65\columnwidth]{images/whyD} & \includegraphics[width=0.65\columnwidth]{images/whytau} \\
    (a) Online job optimization & (b) Effect of $D$ &  (c) Effect of $\tau$
    \end{tabular}
    \caption{Online Progress Estimation}\label{fig:progress}
	\end{center}
\end{figure*}

\section{Online Progress Estimation} \label{progress}
Given a ML job $J$, the online job optimization framework divides the execution of the job $J$ into two phases,
the initialization phase and the online tuning phase, as shown in Figure~\ref{fig:progress}(a).
After initialization, online job optimization framework preprocesses these collected execution metrics ($\langle j , X_i, \ya, \yb\rangle$, as illustrated in Figure~\ref{fig:d}a)
into triples ($\langle X_i, \loss_i,  Y_i\rangle$, as shown in Figure~\ref{fig:d}b) to train BO, then BO will recommend the next optimal setting in online tuning phase.
In this section, we focus on initialization phase, specifically, how to estimate an accurate remaining completion time $Y_i$ efficiently.

\subsection{Estimation Problem Transformation}\label{transform}
$Y_i$ was defined as the estimated remaining completion time assuming that the remaining iterations will use $X_i$ and start from where the model has reached a loss down to $\loss_i$.
Besides, as discussed in Section ~\ref{tuning}, $Y_i$ is not a direct measurement but a product
\begin{align}\nonumber
    Y_i = \bar{t}(X_i) \times r_j(X_i)
\end{align}

where $\bar{t}(X_i)$ is the average execution time per-iteration of given ML job $J$ at setting $X_i$,
and (ii) $r_j(X_i)$ is estimated number of iterations left to reach convergence of the running ML job $J$.


Take Figure~\ref{fig:d}a as an example, when the model has reached a loss $\loss_{j}$, the ML job switch to setting $X_{i}$ and runs $a$ iterations.
Then we have collected the executed statistics: $\langle j , X_{i}, \ensuremath{t^{j}_i}, \ensuremath{l^{j}_i}\rangle$, $\cdots, \langle j+a, X_i, \ensuremath{t^{j+a}_i}, \ensuremath{l^{j+a}_i}\rangle$.
The average cost per iteration of a given ML job $J$ at setting $X^i$ can be derived by $$\bar{t}(X_i) = \frac{1}{a} \sum_{z = j+1}^{z = j+a} \ensuremath{t^{z}_i}.$$
However, estimating the remaining iterations $r_j(X^i)$ to let ML job $j$ reaches convergence is not as easy as obtaining $\bar{t}(X^i)$ as
(i) convergence-rate analysis is truly difficult~\cite{recht2011hogwild,shalev2014understanding,nemirovski2009robust} even in ML theory,
and (ii) while theoretical analysis can provide upper bounds on the number of iterations required, it is often difficult to translate this to how the algorithm will work in practice for a given ML job $J$.
We drop $X_i$ and $\loss_i$ if the context is clear and denote $r_j(X_i)$ as $r$.


In order to devise an accurate and feasible solution to estimate the remaining iterations $r$, we start to analyze the convergence rates of ML jobs from scratch.
The training phase of a given ML job $J$ is to minimize the convex function $f : \w{} \subseteq \mathbb{R}^n \rightarrow \mathbb{R}$,
more precisely,
\begin{align}\nonumber
  \underset{\w{} \in \mathbb{R}^n}{\text{minimize}} ~~~ f(\w{})
\end{align}

In other words, the training phase ML job is to find a model parameter $\w{}$, which best predicts the label of each given input record.
A popular way to minimize a convex function $f$ is via {\em first-order stochastic} algorithms.
These algorithms can be described by using the following iteration %$\w{}^{j+1} \leftarrow \w{}^j - \eta \nabla f(\w{}^j)$.
\begin{align}\nonumber
\w{}^{j+1} \leftarrow \w{}^j - \eta \nabla f(\w{}^j)
\end{align}

Generally, we say the ML job $J$ reaches convergence if
\begin{align}\label{eqn:converge}
  f(\w{}^k)-f(\w{}^*) \leq \epsilon
\end{align}
where $\epsilon$ is user-specified loss threshold, $\w{}^*$ is the optimal model parameters, e.g., it can predict the ground truth label for each input record.

In ML theory area, the ML job convergence rate analysis problem is trying to find the number of iterations $k$ such that $\mathbb{E} [f(\w{}^k) - f(\w{}^*)] \leq \epsilon$.
In order to establish convergence rates to the optimal solution, they assume convex function $f$ is $L$-Lipschitz and $m$-strongly convex in theoretically~\cite{nemirovski2009robust,recht2011hogwild}.
If convex function $f$ is $L$-smooth, then
\begin{align} \nonumber
  ||\nabla f(\w{}^a) - \nabla f(\w{}^b)|| \leq L||\w{}^a - \w{}^b||, ~~\forall~~ \w{}^a,\w{}^b \in \mathbb{R}^n,
\end{align}
where $||\cdot||$ denotes the Euclidean norm. Let $\w{}^a = \w{}^k, \w{}^b = \w{}^*$, as proved in \cite{nemirovski2009robust}, we then obtain
\begin{align} \label{eqn:loss}
   f(\w{}^k) - f(\w{}^*) \leq  \frac{L}{2} ||\w{}^k - \w{}^*||^2, ~~\forall~~\w{}^k \in \mathbb{R}^n,
\end{align}
take expectation at both sides, we have
\begin{align} \nonumber
   \mathbb{E} [f(\w{}^k) - f(\w{}^*)] \leq  \frac{L}{2} \mathbb{E} [||\w{}^k - \w{}^*||^2]
\end{align}

Let $\frac{L}{2} \mathbb{E} [||\w{}^k - \w{}^*||^2] \leq \epsilon$, thus we can transform ML job convergence criteria in Equation~(\ref{eqn:converge}) to
\begin{align} \label{eqn:newobj}
    & \mathbb{E} [f(\w{}^k) - f(\w{}^*)]  \leq  \frac{L}{2} \mathbb{E} [||\w{}^k - \w{}^*||^2] \leq \epsilon
\end{align}
Thus, if we can find the model parameter $\w{}^k$, which satisfies $\mathbb{E} [||\w{}^k - \w{}^*||^2] \leq \frac{2}{L} \epsilon$, then we can conclude the ML job is convergence.

Through this, we can track the algorithmic progress and establish convergence rates to the optimal solution by the model parameter iterations.
Specifically, consider ML job $J$ switch to setting $X_i$ when the loss is $\loss_j$, the remaining iterations $r$ estimation is trying to find the number of iterations,
which update $\w{}^j$ to $\w{}^k$ as follows.
\begin{align} \label{eqn:ssgd}
& \w{}^{j+1} = \w{}^j-\eta \nabla f(\w{}^j)  \\ \nonumber
& \w{}^{j+2} = \w{}^j-\eta \nabla f(\w{}^j) - \eta \nabla f(\w{}^{j+1})  \\ \nonumber
& \cdots \\ \nonumber
& \w{}^{k} = \w{}^j-\eta \nabla f(\w{}^j) - \eta \nabla f(\w{}^{j+1})  - \cdots - \eta \nabla f(\w{}^{j+r})
\end{align}


By exploiting the theoretical results and collected execution metrics,
we propose stateless estimation and stateful estimation approaches in Section~\ref{sec:stateless} and ~\ref{sec:stateful}, respectively.

\subsection{Stateless Estimation}\label{sec:stateless}

In theory literatures, there are many research works~\cite{meng2017convergence,recht2011hogwild,shalev2014understanding,nemirovski2009robust} analyzed the convergence rate of various machine learning algorithms.
For instance, classical machine learning models, like logistic regression and SVM with $l_2$ regularization, the loss function $f$ is $L$-smooth and strongly convex.
Under these assumptions, they concluded $O(\frac{1}{\loss})$-rate of convergence with theoretical analysis for serial Stochastic Gradient Decent algorithms.
i.e., after $k \geq \frac{L\alpha}{\epsilon}$ iterations, we arrived $\mathbb{E} [f(\w{}^k) - f(\w{}^*)] \leq \epsilon$.
This theoretical upper bound also was used in \cite{gdoptimizer} to estimate the total number of iterations required by different Gradient Descent algorithms over sampled training statistics.

This theoretical bound $O(\frac{1}{\loss})$-rate cannot be applied to our problem directly, as this convergence rate was based on serial SGD algorithms.
However, our problem is employing parallelized Stochastic Gradient Descent algorithms inherently.
Fortunately, Hogwild!~\cite{recht2011hogwild} proposed a novel theoretical analysis to parallelizing SGD algorithms,
the convergence rate of parallelizing SGD algorithms was concluded as,
after $k \geq O(\frac{1}{\epsilon}\log(\frac{1}{\epsilon}))$ iterations, we arrived $\mathbb{E} [f(\w{}^k) - f(\w{}^*)] \leq \epsilon$, adopted from Proposition 4.1 in \cite{recht2011hogwild}.

As shown in Figure~\ref{fig:progress}(b), consider a ML job $J$ switch to setting $X_i$ when the loss is down to $l_j$,
then job $J$ run $a$ iterations, thus we have $r$ quadruples $\{ \langle j+1 , X_i, \ensuremath{t^{j+1}_i}, \ensuremath{l^{j+1}_i}\rangle, \cdots, \langle j+a, X_i, \ensuremath{t^{j+a}_i}, \ensuremath{l^{j+a}_i}\rangle \}$.
Then consider the theoretical bound of $O(\frac{1}{\loss}\log(\frac{1}{\loss}))$ convergence rate, 
as $\log(\frac{1}{\epsilon})$ will be negative value if the observed loss is large than 1, we used a constant $D \geq LD_0$, with $D_0 = ||\w{}^0 - \w{}^*||$, to avoid such cases.
Thus, we could estimate its remaining iterations $r$ by

\begin{enumerate}
  \item Fit the function $\frac{\alpha_i}{\loss}\log(\frac{D}{\loss})$
   by using $\{\langle j+1 ,\ensuremath{l^{j+1}_i}\rangle, \cdots, \langle j+a, \ensuremath{l^{j+a}_i}\rangle\}$ to learn the value of $\alpha_i$.
  We then can plot the convergence rate curve as the dotted line in Figure~\ref{fig:progress}(b).
  \item Estimate the total number of iteration by set $\loss = \epsilon$, i.e., $k = \lfloor \frac{\alpha_i}{\epsilon}\log(\frac{D}{\epsilon}) \rfloor$.
  \item Compute the remaining iterations by $r = k - (j+a)$.
\end{enumerate}


Through this way, we can derive $Y_i$ by $\bar{t}(X_i) \times r$, then we can estimate the remaining completion time $Y_i$ for each $X_i$ and $\loss_i$ pair.
This approach is simple but ineffective as (i) it is stateless, as it does not take the current loss $\loss_i$ into consideration,
(ii) $\alpha_i$ has several hidden parameters, as we will show it shortly, which will be affect by the system setting $X_i$ significantly.

\subsection{Stateful Estimation}\label{sec:stateful}
In order to address the above issues in stateless approach, we propose stateful approach in this section.
It exploits the current model loss $\loss_i$ and setting $X_i$ to estimate a more accurate $r$.

As Proposition 4.1 in \cite{recht2011hogwild} stated, after $k \geq \frac{\alpha}{\epsilon}\log(\frac{LD_0}{\epsilon})$, we have $\mathbb{E} [f(\w{}^k) - f(\w{}^*)] \leq \epsilon$.
Here, the analysis assume that the job start at model parameter $\w{}^0$, however, in our problem, the parallelizing SGD algorithm always restart at a specific model parameter $\w{}^j$,
with known loss $\loss_j$, thus, our first improvement is exploiting Lemma~\ref{lem:lossj} to polish the fit function in above procedures.

\begin{lemma}\label{lem:lossj}
\begin{align}\nonumber
  \frac{\alpha_i}{\loss}\log(\frac{D}{\loss}) \geq \frac{\alpha_i}{\loss}\log(\frac{LD_j}{\loss}) \\ \nonumber
  \frac{\alpha_i}{\loss}\log(\frac{LD_j}{\loss}) \geq \frac{\alpha_i}{\loss}\log(\frac{\loss_j}{\loss})
\end{align}
\end{lemma}

\begin{proof}
\begin{align} \nonumber
 & D \geq L D_0 = L ||\w{}^0 - \w{}^*||^2   \\  \nonumber
 & ||\w{}^0 - \w{}^*||^2 \geq ||\w{}^j - \w{}^*||^2 = D_j~~\text{is always true} \\ \nonumber
 & L||\w{}^j - \w{}^*||^2 \geq f(\w{}^j) - f(\w{}^*)~~\text{by Equation~(\ref{eqn:loss})} \\ \nonumber
 & \loss_j = f(\w{}^j) - f(\w{}^*)~~\text{by $\loss_j $Definition} \\ \nonumber
 & \text{thus, we have}~~ D \geq L D_j \geq \loss_j
\end{align}
In addition, $\log(\frac{1}{\loss})$ is monotonic increasing, plugging above conclusion into $\log(\frac{1}{\loss})$ completes the proof. 
\end{proof}

With Lemma~\ref{lem:lossj}, we could refine the fit function to $\frac{\alpha_i}{\loss}\log(\frac{l_j}{\loss})$, which could estimate a more accurate remaining iteration $r$.
As shown in Figure~\ref{fig:progress}(b), according to the same collected statistics (i.e., $\{\langle j+1 , X_i, \ensuremath{t^{j+1}_i}, \ensuremath{l^{j+1}_i}\rangle, \cdots, \langle j+a, X_i, \ensuremath{t^{j+a}_i}, \ensuremath{l^{j+a}_i}\rangle \}$),
$k_{D}$ is obviously large than $k_{\loss_j}$, thus $k_{\loss_j} - (j+a) \leq k_{D} - (j+a)$.


Our second improvement is taking the system setting $X_i$ into consideration. 
As the convergence analysis of parallel SGD in~\cite{recht2011hogwild,mania2015perturbed}, 
the difference between parallel SGD and serial SGD is how to update the parameter model $\w^{}$.

Take Figure~\ref{fig:progress}(c) as an example, suppose the setting $X_1$ only has one worker (i.e., it is serial SGD algorithm essentially),
thus the model parameter $\w{}^a$ will update to $\w{}^k$ one by one, as explained in Equation~(\ref{eqn:ssgd}), Section \ref{transform}. 

However, consider the setting $X_2$, it has more than one worker (i.e., it is parallel SGD algorithm), 
the model parameter $\w{}^{2a}$ will not update to $\w{}^k$ one by one, however, it updates as follows,
\begin{align} \nonumber
& \w{}^{2a+1} = \w{}^{2a}-\eta \nabla f(\hat{\w{}}^{2a})  \\ \nonumber
& \w{}^{2a+2} = \w{}^{2a}-\eta \nabla f(\hat{\w{}}^{2a}) - \eta \nabla f(\hat{\w{}}^{2a+1})  \\ \nonumber
& \cdots \\ \nonumber
& \w{}^{k} = \w{}^{2a}-\eta \nabla f(\hat{\w{}}^{2a}) - \eta \nabla f(\hat{\w{}}^{2a+1})  - \cdots - \eta \nabla f(\hat{\w{}}^{2a+r})
\end{align}

where $\hat{\w{}}^{j} = \w{}^{j} + n^j$, and $n^j$ is a stochastic error term.
Observe that all but the initial ($\w{}^{2a}$) and the last ($\w{}^k$) of these iterates might not be an actual time when they exist in the shared memory 
during the asynchronous parallelizing SGD execution.
However $\w{}^{2a}$ is what is stored before the execution starts, and $\w{}^k$ is exactly what is stored at the end of execution.

\cite{mania2015perturbed} propose {\em bounded overlaps} to measure the effect of stochastic error term, {\em bounded overlap} is the lag between a gradient is computed at step $i$ and
when it is used in step $j$, is always less than or equal to $\tau$, i.e., $j-i \leq tau$.

As proofed in ~\cite{leblond2016asaga}, $g(\tau) = 1+6 p_0 \tau + 6 p_1 \tau^2$, where $p_1$ and $p_2$ are constant parameters.
Obviously, different settings $x_i$ should have different $\tau$ values, instead of one universal $\tau$,
Generally, $\tau$ is proportional to the number of workers $n$ in setting $X_i$, thus, we set $\tau = n$,
as shown in Figure~\ref{fig:progress}(c), the fit function at $X_2$ should be $\frac{cg(\tau_2)}{\epsilon}\log(\frac{\loss_{3a}}{\epsilon})$, 
instead of the same setting as $X_1$, i.e., $\frac{cg(\tau_1)}{\epsilon}\log(\frac{\loss_{3a}}{\epsilon})$.






==> 0-Progress.tex <==
%!TEX root = 0-paper.tex



\section{Online Progress Estimation} \label{progress}

One key input to the online job optimization framework is
the estimated remaining completion time $Y_i$,
assuming that the $j$-th iteration has just finished,
the current model has a loss of $l_j$,
and the remaining iterations will continue to use setting $X_i$.

Estimating $Y_i$ has to base on both the collected quadruples $\langle j , X_i, \ya, \yb\rangle$ and statistical progress estimation techniques.
More specifically, $Y_i$ can be estimated as:

$$Y_i = \bar{t_i} \times r_j$$

\noindent
which is a product between (i) \emph{per-iteration execution time} $\bar{t_i}$ (hardware efficiency)
and (ii) \emph{estimated number of iterations left} $r_j$ (statistical progress).
$\bar{t_i}$ could be directly computed as the average of the recorded iteration times of using that setting $X_i$, e.g., $\bar{t_1}$ can be computed as $(t^5_1+ t^6_1 + \cdots + t^9_1)/5$ in Figure~\ref{fig:d}a.
%$Y_1$ in Figure~\ref{fig:d}b is estimated based on the five quadruples $\langle 5, X_1, t^5_1, \l^5_1\rangle$  to $\langle 9, X_1, t^9_1, \l^9_1\rangle$
In this section, we present two approaches to obtain $r_j$, the remaining number of iterations required to reach model convergence.




\subsection{Stateless Progress Estimation}\label{sec:stateless}
The machine learning community has well studied the convergence properties of various machine learning algorithms
\cite{meng2017convergence,RechtRWN11nips,shalev2014understanding,nemirovski2009robust}.
For instance,
if the learning function $f$ is strongly convex and $L$-smooth\footnote{
A convex function $f$ is $L$-smooth when
$  ||\nabla f(\w{}^a) - \nabla f(\w{}^b)|| \leq L||\w{}^a - \w{}^b||, ~~\forall~~ \w{}^a,\w{}^b \in \mathbb{R}^n$,
where $||\cdot||$ denotes the Euclidean norm and $\nabla  f(\w{})$ denotes the gradient of function $f: \mathbb{R}^d \rightarrow \mathbb{R}$ at $\w$.
}, then the convergence rate of {\bf serial} SGD is $O(\frac{1}{\epsilon})$ \cite{nemirovski2009robust},
where $\epsilon$ is the user-specific convergence threshold.
More specifically,
referring to Eq. \ref{loss},
if $\yb \le \epsilon$, then the model is regarded as converged.
In other words,
let $k$ be the total number of iterations required to reach a loss $\epsilon$,
then $k \ge \frac{\mathcal{H_1}}{\epsilon}$, where ${\mathcal{H_1}}$ is the  hidden constant in  $O(\frac{1}{\epsilon})$.

So far, all convergence analysis are based on an \emph{offline} setting:
(1) %, meaning the value $k$ is analyzed under a setting where
the learning {\bf always} starts from an initial model whose parameter $\w^0$ which are {all 0's} in theoretical analysis \cite{shalev2014understanding}; 
and (2) the system setting never changes in the course of the job.
A recent work \cite{gdoptimizer} has leveraged the above to predict the actual value of $k$ by establishing an offline tuning session like iTuned and OtterTune.
First, the losses of some iterations of an ML job are collected, e.g., $\langle 0, l^0 \rangle, \langle 1, l^1\rangle, \langle 2, l^2\rangle, \cdots$.
Then those $\langle j, l^j \rangle$ pairs are fitted to a function $j = \frac{\mathcal{H_1}}{l^j}$ to deduce $\mathcal{H_1}$.
Finally, $k$, the number of iterations that a new ML job required to converge to a loss $\epsilon$ is derived as $k = \frac{\mathcal{H_1}}{\epsilon}$.

We can extend the approach above to online predict $r_j$.
For example, if we also focus on SGD, then we
(i) use the convergence rate of {\bf parallel} SGD instead of that of serial SGD
and
(ii) use only the losses collected during the iterations related to the current setting of interest, $X_i$, to do the fitting.
Specifically,
the convergence rate of parallel SGD
can be represented by the function
\begin{equation}\label{predict}
j = \frac{\mathcal{H_2}}{\yb}\log\frac{d}{\yb}
\end{equation}

\noindent
where $d$ is any constant greater than $Ld_0$, with $d_0 = ||\w{}^0 - \w{}^*||^2$ and $L$ is the Lipschitz constant \cite{RechtRWN11nips}.
Since $\w^*$ is unknown until the training is done, $Ld_0$ becomes a hidden constant $d$
that has to be greater than \yb, or else the log inside the fitting function becomes negative.
Recall from Eq. \ref{loss} that \yb can be arbitrary large.
So the off-the-shelf safest way is to set $d$ as the maximum value in domain.

%is $O(\frac{1}{\epsilon}\log(\frac{1}{\epsilon}))$
Although correct, we regard this approach only as a baseline
because the resulting  estimates would not  be  that reliable
---
(i) the large $d$ would dominate the fitting function even after the log
and
(ii) $d$ is static in a way that would not get tighten even with the update of the model state.
More specifically, $d$ is static because it is stateless --- it is always $L$ times the constant distance between the initial model $\w^0$ and the optimal model $\w^*$ (c.f. $d_0 = ||\w{}^0 - \w{}^*||^2$).
That explains why we name this approach a \emph{stateless} approach.
In Section \ref{sec:stateful} up next, we present a \emph{stateful} approach that takes the latest model state into account so that the value $d$ keeps tighten as the model approaches convergence,
resulting in far more accurate estimations.

%meaning, $k$, the number of iterations to converge if the learning starts from anew, is
% $k \ge O(\frac{1}{\epsilon}\log\frac{1}{\epsilon})$.
%Following the same logic as  \cite{gdoptimizer},
%then we can use the $\langle j, l^j_i \rangle$ pairs collected in the execution metrics from iterations using $X_i$
%to fit a function
%%where $\mathcal{H_2}$ is the hidden constant that we want to deduce from the data and $d$ is any constant greater than
%%for any possible $\yb$ (otherwise the log would be negative).
%where $\mathcal{H_2}$ is the hidden constant that we want to deduce from the data and $d$ is any constant greater than $Ld_0$ where $d_0 = ||\w{}^0 - \w{}^*||^2$, according to ~\cite{recht2011hogwild}.
%%(otherwise the log would be negative).


%What shall be the value of $d$ exactly?
%We treat this as a baseline approach

As a summary, $r_j$ is estimated by:
(i) fitting the function $j = \frac{\mathcal{H_2}}{\yb}\log\frac{d}{\yb}$
using $\yb$ from iterations of using $X_i$ and determine the value of $\mathcal{H_2}$.
Referring to Figure \ref{fig:d}a as an example,
after the j=9-th iteration, we can fit $\langle 5, l^5_1\rangle$ to $\langle 9, l^9_1\rangle$ to determine the constant $\mathcal{H_2}$ specifically for setting $X_1$.
(ii) Substitute \yb with the value $\epsilon$ to the fitting function
and regard the result as $k$,
i.e., $k = \frac{\mathcal{H_2}}{\epsilon}\log\frac{d}{\epsilon}$.
(iii) Since $k$ is an estimated value about the {\bf total} number of iterations required
but in fact $j$ iterations have been elapsed,  we set $r_j= k-j$.




\subsection{Stateful Progress Estimation}\label{sec:stateful}

Our goal now is to derive a better value of $d$ for Eq. \ref{predict} to satisfy two requirements:

%{\noindent
%(R1) $\frac{d}{l_i^j} > 1$; otherwise $\log\frac{d}{\yb}$ is negative.\\
%(R2) $d$ is tighter; specifically, gets tighten with the model updates.
%}
\begin{itemize}
\item (R1) $\frac{d}{l_i^j} > 1$; otherwise $\log\frac{d}{\yb}$ is negative.
\item (R2) $d$ is tighter than $Ld_0$; hopefully, gets tighten with the model updates.
\end{itemize}


%In the following, we show that when \yb's are observed, we can
In the following, we show that  we can
satisfy both (R1) and (R2) by setting $d = \loss_i$,
where $\loss_i$ is the observed loss of the first iteration of using setting $X_i$ (c.f. Section \ref{bo}):

\begin{enumerate}
\item $\yb = f(\w{}^j) - f(\w{}^*)$ \hfill by Eq. \ref{loss}

\item $f(\w{}^j) - f(\w{}^*) \leq  \frac{L}{2} ||\w{}^j - \w{}^*||^2$ \verb|      |by \cite{RechtRWN11nips}, which upper bound the loss.

\item $\mathbb{E}[||\w{}^j - \w{}^*||^2] \leq  \mathbb{E}[||\w{}^0 - \w{}^*||^2]$ \verb|   | by \cite{RechtRWN11nips}, which expects the model parameter $\w^j$
of any executed iteration is closer to the optimal $\w^*$ than  the initial model $\w^0$.

\item Take expectation on both sides of (2), and then combine that with (3), we have:

$$\mathbb{E}[f(\w{}^j) - f(\w{}^*)] \leq  \frac{L}{2} \mathbb{E}[||\w{}^j - \w{}^*||^2] \leq \frac{L}{2}\mathbb{E}[||\w{}^0 - \w{}^*||^2]  =
\frac{L}{2}d_0 \le Ld_0$$

\item Take expectation on both sides of (1), and then  combine that with (4), we have:
%$$\yb \leq \mathbb{E}[f(\w{}^j) - f(\w{}^*)]  \le Ld_0$$
$$\mathbb{E}[\yb] = \mathbb{E}[f(\w{}^j) - f(\w{}^*)]  \le Ld_0, ~~\forall j=ia+z,~~\forall z \in [1,a)$$

\item Now, consider another view of (2):
$$\mathbb{E}[f(\w{}^j) - f(\w{}^*)]  \geq \mathbb{E}[f(\w{}^{j+z}) - f(\w{}^*)], ~~~\forall z>0$$
then we can regard:
%$$\loss_i \geq l_i^j, ~~\forall i \in [1,a]$$
$$\mathbb{E}[\loss_i] \geq \mathbb{E}[l_i^{j}], ~~\forall j=ia+z,~~\forall z \in [1,a)$$

which follows \cite{nemirovski2009robust} to assume the loss of the first iteration of using setting $X_i$ is expected to be larger than the loss of the subsequent iterations and more importantly:

$$\frac{\mathbb{E}[\loss_i]}{\mathbb{E}[l_i^j]} \ge 1$$

\end{enumerate}

So, during online tuning, we can set $d=\loss_i$, it satisfies (R1) by (6) and
satisfies (R2) by (5).  As a result, the fitting function now becomes:

\begin{equation}\label{stateful1}
j = \frac{\mathcal{H_2}}{\yb}\log\frac{\loss_i}{\yb}
\end{equation}



Referring to Figure \ref{fig:d}a as an example again
and assume $l^5_1$ to $l^9_1$ are 0.9, 0.8, 0.7, 0.6, 0.5 respectively.
Then, after the j=9-th iteration, we fit $\langle 5, 0.9 \rangle$ to $\langle 9, 0.5 \rangle$ to determine the constant $\mathcal{H_2}$ using $\loss_i=0.9$.





%\begin{figure*}[ht]
%	\begin{center}
%%    \begin{tabular}{ccc}
%%    \includegraphics[width=0.65\columnwidth]{images/online_1} & \includegraphics[width=0.65\columnwidth]{images/whyD} & \includegraphics[width=0.65\columnwidth]{images/whytau} \\
%%    (a) Online job optimization & (b) Effect of $D$ &  (c) Effect of $\tau$
%    \begin{tabular}{cc}
% \includegraphics[width=\columnwidth]{images/whyD} & \includegraphics[width=\columnwidth]{images/whytau} \\
%      (a) Stateful vs. Stateless &  (b) Effect of $\tau$
%        \end{tabular}
%    \caption{Estimating the total number of iterations}\label{fig:progress}
%	\end{center}
%\end{figure*}

We call this approach a \emph{stateful} approach because the estimation of $k$ now takes into account the model state $\loss_i$ instead of the constant initial state.
Figure \ref{fig:progress}a visualizes the importance of turning the fitting function from stateless (using $d$ in the log)
to stateful (using $\loss_i$ in the log), where the online prediction of $k$ could yield a significant difference.

\begin{figure}[ht]
	\begin{center}
		%    \begin{tabular}{ccc}
		%    \includegraphics[width=0.65\columnwidth]{images/online_1} & \includegraphics[width=0.65\columnwidth]{images/whyD} & \includegraphics[width=0.65\columnwidth]{images/whytau} \\
		%    (a) Online job optimization & (b) Effect of $D$ &  (c) Effect of $\tau$
		\begin{tabular}{c}
			\includegraphics[width=7cm]{images/whyD}
		\end{tabular}
		\caption{Statistical progress estimation: stateful vs. stateless}\label{fig:progress}
	\end{center}
\end{figure}


%{\bf ++++++++++++++++++++++ERIC stops here}
%
%
%{\bf +++ Bo for bounded overlaps +++}
%
%(1) Current fit function:  $j = \frac{\mathcal{H_2}}{\yb}\log\frac{\loss_i}{\yb}$
%
%(2) Drawback: it does not consider system setting $X_i$ explicitly, however, $X_i$ affects {\em statistical efficiency} and {\em hardware efficiency} significantly.
%
%(3) In parallel SGD analysis, they used {\bf bounded overlaps $\tau$} to capture the effect of system setting.
%
%(4) {\bf bounded overlaps} is the lag between a gradient is computed at step $i$ and when it is used in step $j$, is always less than or equal to $\tau$, i.e., $j-i \leq tau$.
%
%(5) $\tau$ is a proxy for the number of workers, it is proportional to the number of workers.
%
%(6) SGD model parameter updates (take Figure~\ref{fig:progress}(b) as an example):
%\begin{align} \nonumber
%& \w{}^{2a+1} = \w{}^{2a}-\eta \nabla f(\hat{\w{}}^{2a})  \\ \nonumber
%& \w{}^{2a+2} = \w{}^{2a}-\eta \nabla f(\hat{\w{}}^{2a}) - \eta \nabla f(\hat{\w{}}^{2a+1})  \\ \nonumber
%& \cdots \\ \nonumber
%& \w{}^{k} = \w{}^{2a}-\eta \nabla f(\hat{\w{}}^{2a}) - \eta \nabla f(\hat{\w{}}^{2a+1})  - \cdots - \eta \nabla f(\hat{\w{}}^{2a+r})
%\end{align}
%where $\hat{\w{}}^{j} = \w{}^{j} + n^j$, and $n^j$ is a stochastic error term.
%Observe that all but the initial ($\w{}^{2a}$) and the last ($\w{}^k$) of these iterates might not be an actual time when they exist in the parameter server during the asynchronous parallelizing SGD execution.
%
%(7) when $\tau = 0$, asynchronous parallelizing SGD is serial SGD.
%when $\tau >0$, the stochastic error term $n^j$ is:
%$n^j = \hat{\w{}}^j - \w{}^j = \sum_{i = j-\tau, i \neq j }^{j+\tau} \eta \nabla f(\hat{\w{}}^j)$
%
%(8) $\tau$ is small, the stochastic error term $n_j$ is small
%
%(9) We consider the effect of $\tau$ explicitly, $j = \frac{\mathcal{H_2^{'} g(\tau_i)}}{\yb}\log\frac{\loss_i}{\yb}$, where $\tau_i$ is the bounded overlap value in setting $X_i$,
%$g(\tau_i) = 1+6 \gamma \tau_i + 4 \gamma \delta^{\frac{1}{2}} \tau_i^2$, where $\gamma$ is the step size, $\delta$ is the maximum frequency that any feature appears in input records~\cite{recht2011hogwild}.
%
%(10) for each training data with setting $X_i$, we first set $\tau_i = \lambda n$ ($n$ is the number of works in setting $X_i$, we set $\lambda = \frac{1}{4}$), then fit function in (9)
%
%(11) Show XX's figure about the effect of consider $X_i$ (i.e., show as $g(\tau_i)$ in fit function)
%
%{\bf ++++ Bo ends here ++++}
%{\bf  +++++++++Notes from Bo +++++++++++}
%$$j = \frac{\mathcal{H_2}}{\yb}\log\frac{d}{\yb}$$
%where $d=Ld_0$ is big, static.
%
%Objective. we want to deduce a correct  and good $d$ that satisfy the 2 requirements:
%
%(R1)
%
%(R2) $d$ is tighter.
%
%
%We find such $d$ as  follows:
%On one hand,
%
%(1) $\yb = f(\w{}^j) - f(\w{}^*)$ by definition
%
%(2) $f(\w{}^j) - f(\w{}^*) \leq  \frac{L}{2} ||\w{}^j - \w{}^*||^2$ by ref
%
%(3) $\mathbb{E}[||\w{}^j - \w{}^*||^2] \leq  \mathbb{E}[||\w{}^0 - \w{}^*||^2]$ by theory, I used the expectation for more easy to concise.
%
%(4) take expectation of (2) at both sides, then substitute (3)  to it, we have  $\mathbb{E}[f(\w{}^j) - f(\w{}^*)] \leq  \frac{L}{2} \mathbb{E}[||\w{}^j - \w{}^*||^2] \leq \frac{L}{2}\mathbb{E}[||\w{}^0 - \w{}^*||^2]  =
%\frac{L}{2}d_0 \le Ld_0$
%
%(5) take expectation of (1) at both sides, then substitute it to (4), we have $\yb \leq \mathbb{E}[f(\w{}^j) - f(\w{}^*)]  \le Ld_0$
%
%On the other hand,
%
%(a) $\mathbb{E}[f(\w{}^j) - f(\w{}^*)]  \geq \mathbb{E}[f(\w{}^{j+i}) - f(\w{}^*)]~~\forall i>0 $ by theory
%
%(b) by (a) and by the defintion of $\loss_i$, we have $\loss_i \geq l_i^j, ~~\forall i \in [1,a]$
%
%(c) We set $d=\loss_i$, it satisfies (R1) $\frac{d}{l_i^j} > 1$ by  (b), and (R2) $d$ is tighter since $\loss_j \le Ld_0$ by (5).
%
%Example, collected statistics $\langle 0, 0.9\rangle$, $\langle 1, 0.8\rangle$, $\langle 2, 0.6\rangle, \langle 3, 0.55\rangle$,
%thus $\loss_j = 0.9$, and the function is
%$$j = \frac{\mathcal{H_2}}{\yb}\log\frac{0.9}{\yb}$$
%fit this function by the collected statistics.
%
%Then shown XX figure to illustrate the effect of $d$.
%
%
%{\bf Bo ends here}


%
%
%
%$$   \mathbb{E} [f(\w{}^0) - f(\w{}^*)] \leq  \frac{L}{2} \mathbb{E} [||\w{}^0 - \w{}^*||^2]  $$
%
%next, we have
%==>
%
%$$   \mathbb{E} [f(\w{}^0) - f(\w{}^*)] \leq  \frac{L}{2} \mathbb{E} [d_0]  $$
%
%
%
%
%
%
%
%
%
%
%
%
%\begin{equation}\label{eqn:converge}
%  f(\w{}^k)-f(\w{}^*) \leq \epsilon
%\end{equation}
%
%
%
%
%
%
%In theory literatures, there are many research works~\cite{meng2017convergence,recht2011hogwild,shalev2014understanding,nemirovski2009robust} analyzed the convergence rate of various machine learning algorithms.
%For instance, classical machine learning models, like logistic regression and SVM with $l_2$ regularization, the loss function $f$ is
%Under these assumptions, they concluded $O(\frac{1}{\loss})$-rate of convergence with theoretical analysis for serial Stochastic Gradient Decent algorithms.
%i.e., after $k \geq \frac{L\alpha}{\epsilon}$ iterations, we arrived $\mathbb{E} [f(\w{}^k) - f(\w{}^*)] \leq \epsilon$.
%This theoretical upper bound also was used in \cite{gdoptimizer} to estimate the total number of iterations required by different Gradient Descent algorithms over sampled training statistics.
%
%This theoretical bound $O(\frac{1}{\loss})$-rate cannot be applied to our problem directly, as this convergence rate was based on serial SGD algorithms.
%However, our problem is employing parallelized Stochastic Gradient Descent algorithms inherently.
%Fortunately, Hogwild!~\cite{recht2011hogwild} proposed a novel theoretical analysis to parallelizing SGD algorithms,
%the convergence rate of parallelizing SGD algorithms was concluded as,
%after $k \geq O(\frac{1}{\epsilon}\log(\frac{1}{\epsilon}))$ iterations, we arrived $\mathbb{E} [f(\w{}^k) - f(\w{}^*)] \leq \epsilon$, adopted from Proposition 4.1 in \cite{recht2011hogwild}.
%
%As shown in Figure~\ref{fig:progress}(b), consider a ML job $J$ switch to setting $X_i$ when the loss is down to $l_j$,
%then job $J$ run $a$ iterations, thus we have $r$ quadruples $\{ \langle j+1 , X_i, \ensuremath{t^{j+1}_i}, \ensuremath{l^{j+1}_i}\rangle, \cdots, \langle j+a, X_i, \ensuremath{t^{j+a}_i}, \ensuremath{l^{j+a}_i}\rangle \}$.
%Then consider the theoretical bound of $O(\frac{1}{\loss}\log(\frac{1}{\loss}))$ convergence rate,
%as $\log(\frac{1}{\epsilon})$ will be negative value if the observed loss is large than 1, we used a constant $D \geq LD_0$, with $D_0 = ||\w{}^0 - \w{}^*||$, to avoid such cases.
%Thus, we could estimate its remaining iterations $r$ by
%
%\begin{enumerate}
%  \item Fit the function $\frac{\alpha_i}{\loss}\log(\frac{D}{\loss})$
%   by using $\{\langle j+1 ,\ensuremath{l^{j+1}_i}\rangle, \cdots, \langle j+a, \ensuremath{l^{j+a}_i}\rangle\}$ to learn the value of $\alpha_i$.
%  We then can plot the convergence rate curve as the dotted line in Figure~\ref{fig:progress}(b).
%  \item Estimate the total number of iteration by set $\loss = \epsilon$, i.e., $k = \lfloor \frac{\alpha_i}{\epsilon}\log(\frac{D}{\epsilon}) \rfloor$.
%  \item Compute the remaining iterations by $r = k - (j+a)$.
%\end{enumerate}
%
%
%Through this way, we can derive $Y_i$ by $\bar{t}(X_i) \times r$, then we can estimate the remaining completion time $Y_i$ for each $X_i$ and $\loss_i$ pair.
%This approach is simple but ineffective as (i) it is stateless, as it does not take the current loss $\loss_i$ into consideration,
%(ii) $\alpha_i$ has several hidden parameters, as we will show it shortly, which will be affect by the system setting $X_i$ significantly.
%
%
%
%
%
%
%
%
%Given a ML job $J$, the online job optimization framework divides the execution of the job $J$ into two phases,
%the initialization phase and the online tuning phase, as shown in Figure~\ref{fig:progress}(a).
%After initialization, online job optimization framework preprocesses these collected execution metrics ($\langle j , X_i, \ya, \yb\rangle$, as illustrated in Figure~\ref{fig:d}a)
%into triples ($\langle X_i, \loss_i,  Y_i\rangle$, as shown in Figure~\ref{fig:d}b) to train BO, then BO will recommend the next optimal setting in online tuning phase.
%In this section, we focus on initialization phase, specifically, how to estimate an accurate remaining completion time $Y_i$ efficiently.
%
%\subsection{Estimation Problem Transformation}\label{transform}
%$Y_i$ was defined as the estimated remaining completion time assuming that the remaining iterations will use $X_i$ and start from where the model has reached a loss down to $\loss_i$.
%Besides, as discussed in Section ~\ref{tuning}, $Y_i$ is not a direct measurement but a product
%\begin{align}\nonumber
%    Y_i = \bar{t}(X_i) \times r_j(X_i)
%\end{align}
%
%where $\bar{t}(X_i)$ is the average execution time per-iteration of given ML job $J$ at setting $X_i$,
%and (ii) $r_j(X_i)$ is estimated number of iterations left to reach convergence of the running ML job $J$.
%
%
%Take Figure~\ref{fig:d}a as an example, when the model has reached a loss $\loss_{j}$, the ML job switch to setting $X_{i}$ and runs $a$ iterations.
%Then we have collected the executed statistics: $\langle j , X_{i}, \ensuremath{t^{j}_i}, \ensuremath{l^{j}_i}\rangle$, $\cdots, \langle j+a, X_i, \ensuremath{t^{j+a}_i}, \ensuremath{l^{j+a}_i}\rangle$.
%The average cost per iteration of a given ML job $J$ at setting $X^i$ can be derived by $$\bar{t}(X_i) = \frac{1}{a} \sum_{z = j+1}^{z = j+a} \ensuremath{t^{z}_i}.$$
%However, estimating the remaining iterations $r_j(X^i)$ to let ML job $j$ reaches convergence is not as easy as obtaining $\bar{t}(X^i)$ as
%(i) convergence-rate analysis is truly difficult~\cite{recht2011hogwild,shalev2014understanding,nemirovski2009robust} even in ML theory,
%and (ii) while theoretical analysis can provide upper bounds on the number of iterations required, it is often difficult to translate this to how the algorithm will work in practice for a given ML job $J$.
%We drop $X_i$ and $\loss_i$ if the context is clear and denote $r_j(X_i)$ as $r$.
%
%
%In order to devise an accurate and feasible solution to estimate the remaining iterations $r$, we start to analyze the convergence rates of ML jobs from scratch.
%The training phase of a given ML job $J$ is to minimize the convex function $f : \w{} \subseteq \mathbb{R}^n \rightarrow \mathbb{R}$,
%more precisely,
%\begin{align}\nonumber
%  \underset{\w{} \in \mathbb{R}^n}{\text{minimize}} ~~~ f(\w{})
%\end{align}
%
%In other words, the training phase ML job is to find a model parameter $\w{}$, which best predicts the label of each given input record.
%A popular way to minimize a convex function $f$ is via {\em first-order stochastic} algorithms.
%These algorithms can be described by using the following iteration %$\w{}^{j+1} \leftarrow \w{}^j - \eta \nabla f(\w{}^j)$.
%\begin{align}\nonumber
%\w{}^{j+1} \leftarrow \w{}^j - \eta \nabla f(\w{}^j)
%\end{align}
%
%Generally, we say the ML job $J$ reaches convergence if
%\begin{align}\label{eqn:converge}
%  f(\w{}^k)-f(\w{}^*) \leq \epsilon
%\end{align}
%where $\epsilon$ is user-specified loss threshold, $\w{}^*$ is the optimal model parameters, e.g., it can predict the ground truth label for each input record.
%
%In ML theory area, the ML job convergence rate analysis problem is trying to find the number of iterations $k$ such that $\mathbb{E} [f(\w{}^k) - f(\w{}^*)] \leq \epsilon$.
%In order to establish convergence rates to the optimal solution, they assume convex function $f$ is $L$-Lipschitz and $m$-strongly convex in theoretically~\cite{nemirovski2009robust,recht2011hogwild}.
%If convex function $f$ is $L$-smooth, then
%\begin{align} \nonumber
%  ||\nabla f(\w{}^a) - \nabla f(\w{}^b)|| \leq L||\w{}^a - \w{}^b||, ~~\forall~~ \w{}^a,\w{}^b \in \mathbb{R}^n,
%\end{align}
%where $||\cdot||$ denotes the Euclidean norm. Let $\w{}^a = \w{}^k, \w{}^b = \w{}^*$, as proved in \cite{nemirovski2009robust}, we then obtain
%
%\begin{align} \label{eqn:loss}
%   f(\w{}^k) - f(\w{}^*) \leq  \frac{L}{2} ||\w{}^k - \w{}^*||^2, ~~\forall~~\w{}^k \in \mathbb{R}^n,
%\end{align}
%
%take expectation at both sides, we have
%
%\begin{align} \nonumber
%   \mathbb{E} [f(\w{}^k) - f(\w{}^*)] \leq  \frac{L}{2} \mathbb{E} [||\w{}^k - \w{}^*||^2]
%\end{align}
%
%Let $\frac{L}{2} \mathbb{E} [||\w{}^k - \w{}^*||^2] \leq \epsilon$, thus we can transform ML job convergence criteria in Equation~(\ref{eqn:converge}) to
%\begin{align} \label{eqn:newobj}
%    & \mathbb{E} [f(\w{}^k) - f(\w{}^*)]  \leq  \frac{L}{2} \mathbb{E} [||\w{}^k - \w{}^*||^2] \leq \epsilon
%\end{align}
%Thus, if we can find the model parameter $\w{}^k$, which satisfies $\mathbb{E} [||\w{}^k - \w{}^*||^2] \leq \frac{2}{L} \epsilon$, then we can conclude the ML job is convergence.
%
%Through this, we can track the algorithmic progress and establish convergence rates to the optimal solution by the model parameter iterations.
%Specifically, consider ML job $J$ switch to setting $X_i$ when the loss is $\loss_j$, the remaining iterations $r$ estimation is trying to find the number of iterations,
%which update $\w{}^j$ to $\w{}^k$ as follows.
%\begin{align} \label{eqn:ssgd}
%& \w{}^{j+1} = \w{}^j-\eta \nabla f(\w{}^j)  \\ \nonumber
%& \w{}^{j+2} = \w{}^j-\eta \nabla f(\w{}^j) - \eta \nabla f(\w{}^{j+1})  \\ \nonumber
%& \cdots \\ \nonumber
%& \w{}^{k} = \w{}^j-\eta \nabla f(\w{}^j) - \eta \nabla f(\w{}^{j+1})  - \cdots - \eta \nabla f(\w{}^{j+r})
%\end{align}
%
%
%By exploiting the theoretical results and collected execution metrics,
%we propose stateless estimation and stateful estimation approaches in Section~\ref{sec:stateless} and ~\ref{sec:stateful}, respectively.
%
%\subsection{Stateful Estimation}\label{sec:stateful}
%In order to address the above issues in stateless approach, we propose stateful approach in this section.
%It exploits the current model loss $\loss_i$ and setting $X_i$ to estimate a more accurate $r$.
%
%As Proposition 4.1 in \cite{recht2011hogwild} stated, after $k \geq \frac{\alpha}{\epsilon}\log(\frac{LD_0}{\epsilon})$, we have $\mathbb{E} [f(\w{}^k) - f(\w{}^*)] \leq \epsilon$.
%Here, the analysis assume that the job start at model parameter $\w{}^0$, however, in our problem, the parallelizing SGD algorithm always restart at a specific model parameter $\w{}^j$,
%with known loss $\loss_j$, thus, our first improvement is exploiting Lemma~\ref{lem:lossj} to polish the fit function in above procedures.
%
%\begin{lemma}\label{lem:lossj}
%\begin{align}\nonumber
%  \frac{\alpha_i}{\loss}\log(\frac{D}{\loss}) \geq \frac{\alpha_i}{\loss}\log(\frac{LD_j}{\loss}) \\ \nonumber
%  \frac{\alpha_i}{\loss}\log(\frac{LD_j}{\loss}) \geq \frac{\alpha_i}{\loss}\log(\frac{\loss_j}{\loss})
%\end{align}
%\end{lemma}
%
%\begin{proof}
%\begin{align} \nonumber
% & D \geq L D_0 = L ||\w{}^0 - \w{}^*||^2   \\  \nonumber
% & ||\w{}^0 - \w{}^*||^2 \geq ||\w{}^j - \w{}^*||^2 = D_j~~\text{is always true} \\ \nonumber
% & L||\w{}^j - \w{}^*||^2 \geq f(\w{}^j) - f(\w{}^*)~~\text{by Equation~(\ref{eqn:loss})} \\ \nonumber
% & \loss_j = f(\w{}^j) - f(\w{}^*)~~\text{by $\loss_j $Definition} \\ \nonumber
% & \text{thus, we have}~~ D \geq L D_j \geq \loss_j
%\end{align}
%In addition, $\log(\frac{1}{\loss})$ is monotonic increasing, plugging above conclusion into $\log(\frac{1}{\loss})$ completes the proof.
%\end{proof}
%
%With Lemma~\ref{lem:lossj}, we could refine the fit function to $\frac{\alpha_i}{\loss}\log(\frac{l_j}{\loss})$, which could estimate a more accurate remaining iteration $r$.
%As shown in Figure~\ref{fig:progress}(b), according to the same collected statistics (i.e., $\{\langle j+1 , X_i, \ensuremath{t^{j+1}_i}, \ensuremath{l^{j+1}_i}\rangle, \cdots, \langle j+a, X_i, \ensuremath{t^{j+a}_i}, \ensuremath{l^{j+a}_i}\rangle \}$),
%$k_{D}$ is obviously large than $k_{\loss_j}$, thus $k_{\loss_j} - (j+a) \leq k_{D} - (j+a)$.
%
%
%Our second improvement is taking the system setting $X_i$ into consideration.
%As the convergence analysis of parallel SGD in~\cite{recht2011hogwild,mania2015perturbed},
%the difference between parallel SGD and serial SGD is how to update the parameter model $\w^{}$.
%
%Take Figure~\ref{fig:progress}(c) as an example, suppose the setting $X_1$ only has one worker (i.e., it is serial SGD algorithm essentially),
%thus the model parameter $\w{}^a$ will update to $\w{}^k$ one by one, as explained in Equation~(\ref{eqn:ssgd}), Section \ref{transform}.
%
%However, consider the setting $X_2$, it has more than one worker (i.e., it is parallel SGD algorithm),
%the model parameter $\w{}^{2a}$ will not update to $\w{}^k$ one by one, however, it updates as follows,
%\begin{align} \nonumber
%& \w{}^{2a+1} = \w{}^{2a}-\eta \nabla f(\hat{\w{}}^{2a})  \\ \nonumber
%& \w{}^{2a+2} = \w{}^{2a}-\eta \nabla f(\hat{\w{}}^{2a}) - \eta \nabla f(\hat{\w{}}^{2a+1})  \\ \nonumber
%& \cdots \\ \nonumber
%& \w{}^{k} = \w{}^{2a}-\eta \nabla f(\hat{\w{}}^{2a}) - \eta \nabla f(\hat{\w{}}^{2a+1})  - \cdots - \eta \nabla f(\hat{\w{}}^{2a+r})
%\end{align}
%
%where $\hat{\w{}}^{j} = \w{}^{j} + n^j$, and $n^j$ is a stochastic error term.
%Observe that all but the initial ($\w{}^{2a}$) and the last ($\w{}^k$) of these iterates might not be an actual time when they exist in the shared memory
%during the asynchronous parallelizing SGD execution.
%However $\w{}^{2a}$ is what is stored before the execution starts, and $\w{}^k$ is exactly what is stored at the end of execution.
%
%\cite{mania2015perturbed,recht2011hogwild} propose {\em bounded overlaps} to measure the effect of stochastic error term, {\em bounded overlap} is the lag between a gradient is computed at step $i$ and
%when it is used in step $j$, is always less than or equal to $\tau$, i.e., $j-i \leq tau$.
%
%After shown in  ~\cite{mania2015perturbed}, we have $g(\tau) = 1+6 \gamma \tau + 4 \gamma \delta^{\frac{1}{2}} \tau^2$, where $\gamma$ is the step size, $\delta$ is the maximum frequency that any feature appears in input records.
%Obviously, different settings $x_i$ should have different $\tau$ values, instead of one universal $\tau$.
%Generally, $\tau$ is proportional to the number of workers $n$ in setting $X_i$, thus, we set $\tau = n$,
%as shown in Figure~\ref{fig:progress}(c), the fit function at $X_2$ should be $\frac{cg(\tau_2)}{\epsilon}\log(\frac{\loss_{3a}}{\epsilon})$,
%instead of the same setting as $X_1$, i.e., $\frac{cg(\tau_1)}{\epsilon}\log(\frac{\loss_{3a}}{\epsilon})$.
%
%
%



==> 0-Progress_bck.tex <==
%!TEX root = 0-paper.tex

\begin{figure*}[ht]
	\begin{center}
		\subfigure[Remaining cost estimation]{\label{fig:online}
			\includegraphics[width=0.65\columnwidth]{images/online_1}
		}
		\subfigure[Effect of $D$]{\label{fig:whyd}
			\includegraphics[width=0.65\columnwidth]{images/whyD}
		}
		\subfigure[Effect of $\tau$]{\label{fig:whytau}
			\includegraphics[width=0.65\columnwidth]{images/whytau}
		}
		\caption{Online Progress Estimation}
	\end{center}
\end{figure*}

\section{Online Progress Estimation} \label{progress}


As mentioned in Section~\ref{tuning}, online job optimization framework uses estimated the remaining completion time $Y^i$ with setting $X^i$ at moment $\loss$ as train data for the BO.
In this section, we focus on how to process collected quadruples ($\langle j , X_i, \ya, \yb\rangle$, as illustrated in Figure~\ref{fig:d}a) to the BO training triples ($\langle X_i, \loss_i,  Y_i\rangle$, as shown in Figure~\ref{fig:d}b).


\subsection{Estimation Objective}\label{prog:obj}

We define $Y^i$ as the remaining completion time of the ML job if we switch to  setting $X^i$ where the model has reached a loss down to $\loss_j$
and at moment $j$.
As we mentioned in Section~\ref{tuning}, $Y^i$ is not directly observed but product by
\begin{align}\label{prog:goal}
    Y^i = \bar{t}(X^i) \times R_j(X^i)
\end{align}
where $\bar{t}(X^i)$ is the average cost per iteration of given ML job $J$ at setting $X^i$,
and $R_j(X^i)$ is the remaining iterations to reach convergence for the ML job $J$ at moment $j$.

In online job optimization framework, the ML job at moment $j$ with parameter value $\w{}^j$. It run $r$ iterations at setting $X^i$.
After $r$ iterations, we collected executed statistics: $\langle j+1 , X_i, \ensuremath{t^{j+1}_i}, \ensuremath{l^{j+1}_i}\rangle$,
$\cdots, \langle j+r, X_i, \ensuremath{t^{j+r}_i}, \ensuremath{l^{j+r}_i}\rangle$.
The average cost per iteration of a given ML job $J$ at setting $X^i$ can be derived by $\bar{t}(X^i) = \frac{1}{r} \sum_{z = j+1}^{z = j+r} \ensuremath{t^{z}_i}$.
However, estimating the remaining iterations $R_j(X^i)$ to let ML job $j$ reaches convergence is not as easy as obtaining $\bar{t}(X^i)$ as
(i) convergence-rate analysis is truly difficult~\cite{recht2011hogwild,shalev2014understanding,nemirovski2009robust} even in ML theory,
and (ii) while theoretical analysis can provide upper bounds on the number of iterations required, it is often difficult to translate this to how the algorithm will work in practice for a given ML job $J$.

In order to devise an accurate and feasible solution to estimate the remaining iterations $R_j(X^i)$, we start to analyze the convergence rates of ML jobs from scratch.
The training phase of a given ML job $J$ is to minimize the convex function $f : \w{} \subseteq \mathbb{R}^n \rightarrow \mathbb{R}$,
more precisely,
\begin{align}\label{eqn:mlobj}
  \underset{\w{} \in \mathbb{R}^n}{\text{minimize}} ~~~ f(\w{})
\end{align}

In other words, the training phase ML job is to find a model parameter $\w{}$, which best predicts the label of each given input record.
A popular way to minimize a convex function $f$ is via {\em first-order stochastic} algorithms.
These algorithms can be described by using the following iteration %$\w{}^{j+1} \leftarrow \w{}^j - \eta \nabla f(\w{}^j)$.
\begin{align}\label{eqn:wupdates}
\w{}^{j+1} \leftarrow \w{}^j - \eta \nabla f(\w{}^j)
\end{align}

Generally, we say the ML job $J$ reaches convergence if
\begin{align}\label{eqn:converge}
  f(\w{}^k)-f(\w{}^*) \leq \epsilon
\end{align}
where $\epsilon$ is user-specified loss threshold, $\w{}^*$ is the optimal model parameters, e.g., it can predict the ground truth label for each input record.

In ML theory area, the ML job convergence rate analysis problem is trying to find the number of iterations $k$ such that $\mathbb{E} [f(\w{}^k) - f(\w{}^*)] \leq \epsilon$.
In theoretical, a major advantage of the above first-order iterative formula is that in combination with strong convexity, and smoothness inequalities one can easily track the algorithmic progress and establish convergence rates to the optimal solution~\cite{nemirovski2009robust}.
Specifically, they assume convex function $f$ is $L$-Lipschitz and $m$-strongly convex.
if convex function $f$ is $L$-smooth, then
\begin{align} \label{eqn:L-lipschitz}
  ||\nabla f(\w{}^a) - \nabla f(\w{}^b)|| \leq L||\w{}^a - \w{}^b||, ~~\forall~~ \w{}^a,\w{}^b \in \mathbb{R}^n,
\end{align}
where $||\cdot||$ denotes the Euclidean norm. Let $\w{}^a = \w{}^k, \w{}^b = \w{}^*$, as proved in \cite{nemirovski2009robust}, we then obtain
\begin{align} \label{eqn:fx}
   f(\w{}^k) - f(\w{}^*) \leq  \frac{L}{2} ||\w{}^k - \w{}^*||^2, ~~\forall~~\w{}^k \in \mathbb{R}^n,
\end{align}
take expectation at both sides, we have
\begin{align} \label{eqn:convert}
   \mathbb{E} [f(\w{}^k) - f(\w{}^*)] \leq  \frac{L}{2} \mathbb{E} [||\w{}^k - \w{}^*||^2]
\end{align}

Through this, we can transform ML job convergence criteria in Equation~(\ref{eqn:converge}) to
\begin{align} \label{eqn:newobj}
    & \mathbb{E} [f(\w{}^k) - f(\w{}^*)]  \leq  \frac{L}{2} \mathbb{E} [||\w{}^k - \w{}^*||^2] \leq \epsilon \\
    & \Longleftrightarrow \mathbb{E} [||\w{}^k - \w{}^*||^2] \leq \frac{2}{L} \epsilon
\end{align}

Thus, given ML job $J$ with setting $X^i$ at moment $j$, the remaining iterations $R_j(X^i)$ estimation is trying to find the number of iterations, which update $\w{}^j$ to $\w{}^k$ as follows
%\begin{align} \label{eqn:updates}
%   \underbrace{\overbrace{\w{}^j-\eta \nabla f(\w{}^j)}^{\w{}^{j+1}}- \cdots - \eta \nabla f(\w{}^{j+R_j(X^i)})}_{\w{}^{k}}
%\end{align}

\begin{align} \nonumber
& \w{}^{j+1} = \w{}^j-\eta \nabla f(\w{}^j)  \\ \nonumber
& \w{}^{j+2} = \w{}^j-\eta \nabla f(\w{}^j) - \eta \nabla f(\w{}^{j+1})  \\ \nonumber
& \cdots \\ \nonumber
& \w{}^{j+k} = \w{}^j-\eta \nabla f(\w{}^j) - \eta \nabla f(\w{}^{j+1})  - \cdots - \eta \nabla f(\w{}^{j+r})
\end{align}


By exploiting the theoretical results and collected execution metrics, we devise an accurate and feasible $R_j(X^i)$ estimation approach in Section \ref{prog:sol}.

%\subsection{$R_j(X^i)$ Estimation Approach}\label{prog:sol}

\subsection{Turning asymptotic bound into estimates}\label{prog:sol-1}

In theory literatures, there are many research works~\cite{recht2011hogwild,shalev2014understanding,nemirovski2009robust} analyzed the convergence rate of various machine learning algorithms.
For instance, classical machine learning models, like logistic regression and SVM with $l_2$ regularization, the loss function $f$ is $L$-smooth and strongly convex.
Under these assumptions, they concluded $O(\frac{1}{\loss})$-rate of convergence with theoretical analysis,
i.e., after $k \geq \frac{L\alpha}{\epsilon}$ iterations, we arrived $\mathbb{E} [f(\w{}^k) - f(\w{}^*)] \leq \epsilon$.
This theoretical upper bound also was used in \cite{gdoptimizer} to estimate the total number of iterations required by different Gradient Descent algorithms over sampled training statistics.

\begin{figure}\centering
\includegraphics[width=8cm]{images/estimate_r}
\caption{Collected statistics of $r+mr$ iterations}
\label{fig:collected}
\end{figure}

In our online progress estimation problem, given setting $X^i$ at moment $j$, after $r$ iterations, as shown in Figure~\ref{fig:collected}a, during the initialization, we collected $r$ quadruples $\{ \langle j+1 , X_i, \ensuremath{t^{j+1}_i}, \ensuremath{l^{j+1}_i}\rangle, \cdots, \langle j+r, X_i, \ensuremath{t^{j+r}_i}, \ensuremath{l^{j+r}_i}\rangle \}$.
With the theoretical guarantee of $O(\frac{1}{\loss})$ convergence rate, we could estimate its remaining iterations $R_j(X^i)$ by:
\begin{enumerate}
  \item Fit the function $\frac{\alpha_i}{\loss}$ by using $\{\langle j+1 ,\ensuremath{l^{j+1}_i}\rangle, \cdots, \langle j+r, \ensuremath{l^{j+r}_i}\rangle\}$ to learn the value of $\alpha_i$.
  We then can plot the convergence rate curve as the black line in Figure~\ref{fig:collected}b.
  \item Estimate the total number of iteration by set $\loss = \epsilon$, i.e., it is $\lfloor \frac{\alpha_i}{\epsilon} \rfloor$.
  \item Compute the remaining iterations by $R_j(X^i) = \lfloor \frac{\alpha_i}{\epsilon} \rfloor -  r$.
\end{enumerate}


This approach is simple but ineffective as (i) the theoretical analysis, i.e., $O(\frac{1}{\loss})$ convergence rate, only provide upper bound to the number of iterations required.
It is difficult to capture the algorithm works in practice, (ii) $O(\frac{1}{\loss})$ convergence rate was established upon the serial update $\w{}$ at each iteration, as shown in Figure~\ref{fig:updates}(a).
However, the progress of asynchronous parallel gradient descent algorithms cannot be precisely analyzed using the serial iterative process.
Workers do not read from shared parameters actual iterates $\w{}^j$, as there is no global clock that synchronizes reads or writes while different workers updates variable $\w{}^j$.
Take Figure~\ref{fig:updates}(b) as an example, at start moment $j$, the model parameter is $\w{}^j$, the model parameter updates to $\w{}^{j+3}$ after 3 iterations.
However, it is not equivalent to say $\w{}^{j+3}$ was updated from $\w{}^{j+2}$, as shown in Figure \ref{fig:updates}(b), it was generated by updating $\w{}^j$ due to asynchronous protocol.

\begin{figure}\centering
\includegraphics[width=8cm]{images/updates}
\caption{Iterative $\w{}$ updates}
\label{fig:updates}
\end{figure}

\subsection{Incorporating convergence analysis with estimates}\label{prog:sol}

In order to overcome the ineffective issue of above approach, we propose an more accurate remaining iteration $R_j(X^i)$ estimation approach by
incorporating parallelizing stochastic gradient descent convergence analysis with the collected execution metrics.


As we discussed above, the asynchronous parallelizing gradient descent algorithm does not update $\w{}^*$ as Equation ~(\ref{eqn:updates}).
Inspired by~\cite{mania2015perturbed}, we bring a stochastic error term $n^j$ in each iteration $j$, thus we rewrite Equation ~(\ref{eqn:updates}) as follow
\begin{align} \label{eqn:asynupdates}
    \underbrace{\overbrace{\w{}^j-\eta \nabla f(\w{}^j + n^j)}^{\w{}^{j+1}}- \cdots - \eta \nabla f(\w{}^{j+R_j(X^i)}+ n^{j+R_j(X^i)})}_{\w{}^{k}}
\end{align}
For simplicity $\hat{\w{}}^j = \w{}^j + n^j$, then, we have
\begin{align} \label{eqn:asynupdates}
    \underbrace{\overbrace{\w{}^j-\eta \nabla f(\hat{\w{}}^j)}^{\w{}^{j+1}}- \cdots - \eta \nabla f(\hat{\w{}}^{j+R_j(X^i)})}_{\w{}^{k}}
\end{align}

Observe that all but the initial ($\w{}^j$) and the last ($\w{}^k$) of these iterates might not be an actual time when they exist in the shared memory during the asynchronous parallelizing SGD execution.

\begin{theorem}\label{them:remain}
Given setting $X^i$ at moment $j$, the asynchronous stochastic gradient descent algorithm reaches an accuracy of $\mathbb{E}[f(\w{}^k)-f(\w{}^*)] \leq \epsilon$ after
\begin{align}
  R_j(X^i) = \lfloor \frac{\mathsf{c} g(\tau_i)}{\epsilon} \log(\frac{D_j}{\epsilon}) \rfloor - r
\end{align}
iterations, where $D_j \geq dist(\w{}^0,\w{}^*) - dist(\w{}^j,\w{}^0)$, $g(\tau_i)=1+\tau_i (\delta + \eta) + \tau_i^2 \eta \delta$.
\end{theorem}

Thus, with Theorem~\ref{them:remain}, given setting $X^i$ at moment $j$, we could estimate an more accurate remaining iteration $R_j(X^i)$ by (i) calculating the exact $g(\tau_i)$ at setting $X^i$,
(ii) tighting the distance $D_j$ by exact model parameter $\w{}^j$, and (iii) fitting the constant factor (without effect of parallelizing SGD execution) by collected statistics.

The main idea to proof Theorem \ref{them:remain} is to substitute Equation~(\ref{eqn:bounded-ana-1}, \ref{eqn:bounded-ana-2}) (cf. Lemma~\ref{lem:expection}) to Equation~(\ref{eqn:iter-ana-3}) (cf. Lemma~\ref{lem:aj}), then we solve the recursive of $a_j$ by induction. The proof is shown as follows.

\begin{proof}
TODO
\end{proof}


Let $a_j = \mathbb{E}[||\w{}^{j} -  \w{}^{*}||^2]$, we have
\begin{lemma}[Recursive $a_j$]\label{lem:aj}
\begin{align}\label{eqn:iter-ana-3}
  a_{j+1} & \leq (1-\eta m)a_j  + \eta^2 M^2 + 2\eta m E[||\hat{\w{}}^{j} -  \w{}^{j}||^2] \\ \nonumber
  & + 2 \eta E[(\hat{\w{}}^j - \w{}^j)^T \nabla f(\hat{\w{}}^j)]
\end{align}
\end{lemma}
where $E[||\hat{\w{}}^{j} -  \w{}^{j}||^2]$ captures the effects of stochastic error $n^j$,
$E[(\hat{\w{}}^j - \w{}^j)^T \nabla f(\hat{\w{}}^j)]$ shows the projection of $n^j$ at each step.
%The recursive Equation~(\ref{eqn:iter-ana-3}) is key to our analysis.

\begin{proof}
We start by the iterative analysis of $||\w{}^{j+1} -  \w{}^{*}||^2$.

\begin{align}\label{eqn:iter-ana} \nonumber
\small
  & ||\w{}^{j+1} -  \w{}^{*}||^2  =  || \w{}^j - \eta \nabla f(\hat{\w{}}^j) - \w{}^*||^2 \\ \nonumber
  & =  ||\w{}^{j} -  \w{}^{*}||^2 - 2 \eta (\w{}^j - \w{}^*)^T \nabla f(\hat{\w{}}^j) + \eta^2||\nabla f(\hat{\w{}}^j)||^2\\ \nonumber
  & =  ||\w{}^{j} -  \w{}^{*}||^2 - 2 \eta (\hat{\w{}}^j - \w{}^*)^T \nabla f(\hat{\w{}}^j) + \eta^2||\nabla f(\hat{\w{}}^j)||^2 \\
  & + 2 \eta (\hat{\w{}}^j - \w{}^j)^T \nabla f(\hat{\w{}}^j)
\end{align}

Moreover, since $f$ is $m$-strongly convex, $\forall \w{}^a, \w{}^b$, we know that
\begin{align}\nonumber
 (\w{}^a-\w{}^b)^T(\nabla f(\w{}^a) - \nabla f(\w{}^b)) \geq m ||\w{}^a-\w{}^b||^2
\end{align}

By setting $\w{}^a = \hat{\w{}}^j, \w{}^b=\w{}^*$, we have $\nabla f(\w{}^*) = 0$ and
\begin{align} \label{eqn:bound-1} \nonumber
  & (\hat{\w{}}^j - \w{}^*)^T \nabla f(\hat{\w{}}^j) \geq m ||\hat{\w{}}^j-\w{}^*||^2  \\ \nonumber
   \text{with}&~||\hat{\w{}}^j-\w{}^*||^2 \geq ||\w{}^j-\w{}^*||^2 - ||\hat{\w{}}^j-\w{}^j||^2 \\
   \text{thus}&~(\hat{\w{}}^j - \w{}^*)^T \nabla f(\hat{\w{}}^j) \geq \frac{m}{2} ||\w{}^j-\w{}^*||^2 - m ||\hat{\w{}}^j-\w{}^j||^2
\end{align}

In addition, as a standard assumption~\cite{recht2011hogwild,nemirovski2009robust}, there is a constant $M$ such that
\begin{align}\label{eqn:bound-2}
  || \nabla f(\w{}) || \leq M ~~~\text{almost surely for all}~~~ \w{} \in \mathbb{R}^n
\end{align}

Substituting Equation~(\ref{eqn:bound-1}, \ref{eqn:bound-2}) in Equation~(\ref{eqn:iter-ana}), we have
\begin{align}\label{eqn:iter-ana-2}
  & ||\w{}^{j+1} -  \w{}^{*}||^2 \leq (1-\eta m)||\w{}^{j} -  \w{}^{*}||^2 + 2 \eta m ||\hat{\w{}}^{j} -  \w{}^{j}||^2 \\ \nonumber
  & + \eta^2 M^2 + 2 \eta (\hat{\w{}}^j - \w{}^j)^T \nabla f(\hat{\w{}}^j)
\end{align}

We now take expectation of both side of Equation~(\ref{eqn:iter-ana-2}), then we completes the proof.
\end{proof}

In order to bound $E[||\hat{\w{}}^{j} -  \w{}^{j}||^2]$ and $E[(\hat{\w{}}^j - \w{}^j)^T \nabla f(\hat{\w{}}^j)]$, we introduce parameter bounded overlap $\tau_i$ as follows.

\begin{definition}[Bounded overlaps]
Given setting $X^i$, the lag between when a gradient is computed in step $j$ and when it is used in step $j'$ is defined as bounded overlap $\tau_i$, where $j' - j \leq \tau_i$
\end{definition}
In the case that $\tau_i=0$, this degenerates to serial stochastic gradient descent.


\begin{lemma}\label{lem:expection}
\begin{align}
& E[||\hat{\w{}}^{j} -  \w{}^{j}||^2] \leq \mathsf{c}_1 \eta^2 M^2 (\tau_i + \tau_i^2 \mathsf{\delta} ) \label{eqn:bounded-ana-1} \\
& E[(\hat{\w{}}^j - \w{}^j)^T \nabla f(\hat{\w{}}^j)] \leq  \mathsf{c}_2 \eta M^2 \tau_i \mathsf{\delta} \label{eqn:bounded-ana-2}
\end{align}
where $\delta$ is a constant.
\end{lemma}

\begin{proof}
TODO, The proof of above expectation is similar with Hogwild.
\end{proof}




==> 1-Progress.tex <==
%!TEX root = 0-paper.tex



\section{Online Progress Estimation} \label{progress}

One key input to the online job optimization framework is
the estimated remaining completion time $Y_i$,
assuming that the $j$-th iteration has just finished,
the current model has a loss of $l_j$,
and the remaining iterations will continue to use setting $X_i$.

Estimating $Y_i$ has to base on both the collected quadruples $\langle j , X_i, \ya, \yb\rangle$ and statistical progress estimation techniques.
More specifically, $Y_i$ can be estimated as:

$$Y_i = \bar{t_i} \times r_j$$

\noindent
which is a product between (i) \emph{per-iteration execution time} $\bar{t_i}$ (hardware efficiency)
and (ii) \emph{estimated number of iterations left} $r_j$ (statistical progress).
$\bar{t_i}$ could be directly computed as the average of the recorded iteration times of using that setting $X_i$, e.g., $\bar{t_1}$ can be computed as $(t^5_1+ t^6_1 + \cdots + t^9_1)/5$ in Figure~\ref{fig:d}a.
%$Y_1$ in Figure~\ref{fig:d}b is estimated based on the five quadruples $\langle 5, X_1, t^5_1, \l^5_1\rangle$  to $\langle 9, X_1, t^9_1, \l^9_1\rangle$
In this section, we present the approach to obtain $r_j$, the remaining number of iterations required to reach model convergence.



\subsection{Some Approximations} \label{approximation}
The machine learning community has well studied the convergence properties of various machine learning algorithms
\cite{meng2017convergence,RechtRWN11nips,shalev2014understanding,nemirovski2009robust}.

Recall that in learning, we face the problem of minimizing the empirical risk function
$$F(w) = \frac{1}{n}\sum_{i=1}^{n}f(w, Z_i)$$
Where $n$ is the number of data examples in the whole training dataset $Z$ and $f$ is the loss function for the data example $Z_i \in Z$ with model $w$.

For instance, if the empirical risk function is c-strongly convex\footnote{
If a function $g$ is c-strongly convex, it means that $g(w^a) \ge g(w^b) + (w^a - w^b)^T \nabla g(w^b) + \frac{c}{2}||w^a - w^b||^2, ~~\forall~~ \w{}^a,\w{}^b \in \mathbb{R}^n$, where $||\cdot||$ denotes the Euclidean norm and $\nabla  g(\w{})$ denotes     the gradient of function $g: \mathbb{R}^d \rightarrow \mathbb{R}$ at $\w$. 
}	and L-smooth\footnote{
A convex function $g$ is $L$-smooth when
	$  ||\nabla g(\w{}^a) - \nabla g(\w{}^b)|| \leq L||\w{}^a - \w{}^b||, ~~\forall~~ \w{}^a,\w{}^b \in \mathbb{R}^n$.
}, then \textbf{serial} SGD takes $k\sim O(\frac{1}{\epsilon})$\cite{nemirovski2009robust} iterations to make $\mathbb{E}[F(w^k) - F(w^*)] \le \epsilon$. Where $w^*$ is the optimal model parameter, $w^k$ is the updated model parameter after iteration k and $\epsilon$ is the user-specific convergence threshold. More specifically, if $F(w^k) - F(w^*) \le \epsilon$, then the model is regarded as converged after iteration k. In other words, let $k$ be total number of iterations required to reach a threshold $\epsilon$, then $k \ge \frac{\mathcal{H_1}}{\epsilon}$, where ${\mathcal{H_1}}$ is the hidden constant in $O(\frac{1}{\epsilon})$. However, while the ML systems want to check whether 
the updated model after iteration $j$ is converged, the value of $F(w^j) - F(w^*)$ should be computed, then two difficulties emerge:(1) it will be way too expensive to compute the value of $F(w^j)$, since it will scan the whole training dataset; and (2) the model $w^*$ and $F(w^*)$ are both unknown. Therefore, it is impossible to get the exact value of $F(w^j) - F(w^*)$. Here, we adapt some tricks to approximate it.

The loss of iteration j, \yb (Section: \ref{bo}), can be denoted as:
$$ \yb = \frac{1}{m}\sum_{t=1}^{m}f(w^j, Z_{S_{\alpha,t}^{j}}) $$
%Where $m$ is the number of data examples which are uniformly sampled from the whole dataset within an iteration. 
Where $S_{\alpha}^j$ is a subset of $m$ numbers which are uniformly sampled from $\{1,2,3,...,n\}$ without replacement. Thus, $Z_{S_{\alpha}^j}$ is regarded as a mini-batch of $m$ examples within iteration $j$. And, there can be ${n \choose m}$ different choices with same probability for $S_{\alpha}^j$. 
Then we can denote the expectation of \yb as
$$\mathbb{E}[\yb] = \sum_{\alpha ' = 1}^{{n \choose m}}\frac{1}{{n \choose m}}\frac{1}{m}\sum_{t=1}^{m}f(w^j, Z_{S_{\alpha ',t}^j})$$
$$= \frac{1}{m{n \choose m}}\sum_{t=1}^{n}\frac{m{n \choose m}}{n}f(w^j, Z_t)$$
It is easy to verify that
$$ \mathbb{E}[\yb] = F(w^j)$$
The loss of iteration j, $\yb$, is therefore an unbiased estimate of the empirical risk function $F(w^j)$. And for GD algorithms, $\yb$ can be obtained directly in iteration j with tiny overhead. 

%And in most large-scale machine learning tasks, the value $F(w^*)$ is negligible compared with the user-specific convergence threshold $\epsilon$, since it is efficient to avoid model overfitting with such setting \cite{largescale2016, deeplearning2016}. Hence, $\yb$ is a good approximation of the value $F(w^j) - F(w^*)$. 
When training large models with sufficient representational capacity, we often observe that the loss of the training set $\yb$ decreases steadily over time. However, applying the model which fits the training dataset perfictly(i.e., the result model $w$ is the optimum $w^*$) to the test dataset,
the inference results will often be bad for the test set. We call such situations as overfitting. In oder to avoid overfitting when training, practically, the thresholder $\epsilon$ will be set magnitude larger than the minimal value of empirical risk $F(w^*)$ \cite{largescale2016, deeplearning2016}. Hence, while estimating $F(w^j) - F(w^*)$, it is safe to ignore $F(w^*)$.


Because of above two approximations, $\yb$ is regarded as a good estimate of the value $F(w^j) - F(w^*)$. 
\subsection{Progress Estimation}
So far, all convergence analysis are based on an \emph{offline} setting:
(1) %, meaning the value $k$ is analyzed under a setting where
the learning {\bf always} starts from an initial model whose parameter $\w^0$ which are {all 0's} or random real values which are near {0's}\cite{shalev2014understanding, deeplearning2016}; 
and (2) the system setting never changes in the course of the job.
A recent work \cite{gdoptimizer} has leveraged the above to predict the actual value of $k$ by establishing an offline tuning session like iTuned and OtterTune.
First, the losses of some iterations of an ML job are collected, e.g., $\langle 0, l^0 \rangle, \langle 1, l^1\rangle, \langle 2, l^2\rangle, \cdots$.
Then those $\langle j, l^j \rangle$ pairs are fitted to a function $j = \frac{\mathcal{H_1}}{l^j}$ to deduce $\mathcal{H_1}$.
Finally, $k$, the number of iterations that a new ML job required to converge to a loss $\epsilon$ is derived as $k = \frac{\mathcal{H_1}}{\epsilon}$.

We can extend the approach above to online predict the number of remaining iterations after iteration $j_0$.
For example, if we also focus on SGD, then we
(i) use the convergence rate of {\bf parallel} SGD instead of that of serial SGD 
and
(ii) use only the losses collected during the iterations related to the current setting of interest, $X_i$, to do the fitting.
Specially, when the empirical risk function $F(w)$ is L-smooth, c-strongly convex, for \textbf{asynchronous} parallel SGD\cite{RechtRWN11nips}, the number of remaining iterations after iteration $j_0$ equal to 
$$r_{j_0}(\epsilon) \ge \frac{\mathcal{H_2}}{\epsilon}\log\frac{d}{\epsilon}$$
are sufficient to guarantee that $\mathbb{E}[F(w^{j_0}) - F(w^*)] \le \epsilon$.
Where $d = L||w^{j_0} - w^*||^2$ with L as the Lipschiz constant.

Thus, to estimate the number of iterations left $r_{j_0}$, ${\mathcal{H_2}}$ and $d$ must be determined. Now, suppose that the online tuning program switches to setting $X_i$ in the iteration $j_0$, and then continues training for $a$ iterations. During this period, 
we will collect a set of pairs $\{<j, \yb>\}_{j=j_0}^{j_0+a-1}$. If those pairs are scattered in a 2D space, we can consider they fluctuate around a curve
$$j = j_0 + \frac{\mathcal{H_2}}{\yb}\log\frac{d}{\yb}$$
Where we (i) set $d$ to an appropriate value which satisfies $d \le 2\frac{L}{c}l_{i}^{j_0}$ and (ii) fit pairs $\{<j, \yb>\}_{j=j_0}^{j_0+a-1}$ into this curve to derive $\mathcal{H_2}$. Thereafter, 
we can estimate the remaining number of iterations after the first iteration $j_0$ with setting $X_i$, $r_{j_0} = \frac{\mathcal{H_2}}{\epsilon}\log\frac{d}{\epsilon}$.

Now let us have a brief dissuction on why $d$ should satisfy $d \le 2\frac{L}{c}l_{i}^{j_0}$. 
\begin{enumerate}
\item $l_{i}^{j_0} = F(w^{j_0}) - F(w^*)$ \hfill by Section \ref{approximation}
\item $d = L||w^{j_0} - w^*||^2$ 
\item $||w^{j_0} - w^*||^2 \le \frac{2}{c}(F(w^{j_0}) - F(w^*))$ \verb|	| by \cite{RechtRWN11nips}, since the empirical risk function $F(w)$ is c-strongly convex.
\item $||w^{j_0} - w^*||^2 \ge \frac{2}{L}(F(w^{j_0}) - F(w^*))$ \verb|	| by \cite{RechtRWN11nips}, since the empirical risk function $F(w)$ is L-smooth.

\item Then combine (1), (2) and (3), it is easy to know that
$$d \le \frac{2L}{c}l_{i}^{j_0}$$

\item By the way, consider (3) and (4), we can get the lower bound of $\frac{L}{c}$. 
$$\frac{L}{c} \ge 1$$

\end{enumerate}




